Refinement of Interval Approximations for Fully Commutative Quivers

A fundamental challenge in multiparameter persistent homology is the absence of a complete and discrete invariant. To address this issue, we propose an enhanced framework that realizes a holistic understanding of a fully commutative quiver's representation via synthesizing interpretations obtained from intervals. Additionally, it provides a mechanism to tune the balance between approximation resolution and computational complexity. This framework is evaluated on commutative ladders of both finite-type and infinite-type. For the former, we discover an efficient method for the indecomposable decomposition leveraging solely one-parameter persistent homology. For the latter, we introduce a new invariant that reveals persistence in the second parameter by connecting two standard persistence diagrams using interval approximations. We subsequently present several models for constructing commutative ladder filtrations, offering fresh insights into random filtrations and demonstrating our toolkit's effectiveness in analyzing the topology of materials.

==> legacy/001-invertible-operations.tex <==
\section{Invertible operations on $CL(4)$}

\begin{prop}\label{prop:endo}
Let $\sigma$ be an additive endofunctor of  $\cat{rep}\ Q$ with an inverse $\tau$ such that
\begin{enumerate}
    \item $\sigma$ is an automorphism on $\mathcal{L}$;
\end{enumerate}
Then for each $M\in\cat{rep}\ Q$, the multiplicity function of $M$ satisfies:
\[
d_{\sigma(M)}(L)=d_{M}(\tau(L)).
\]
\begin{proof}
\end{proof}
By Krull-Schmidt theorem, we have
\[
M\cong \Directsum{L\in \mathcal{L}} L^{d_M(L)}.
\]
Since $\sigma$ is additive, we can write
\[
\begin{aligned}
\sigma(M) &\cong \Directsum{L\in \mathcal{L}}\sigma(L)^{d_M(L)}\\
&\cong  \Directsum{\tau(T)\in \mathcal{L}}\sigma(\tau(T))^{d_M(\tau(T))}\ \mbox{\textcolor{blue}{set $L\cong \tau(T)$}}\\
&\cong  \Directsum{T\in \mathcal{L}}T^{d_M(\tau(T))}\\
&\cong  \Directsum{L\in \mathcal{L}}L^{d_M(\tau(L))}.
\end{aligned}
\]
On the other hand, $\sigma(M)\cong \Directsum{L\in \mathcal{L}} L^{d_\sigma(M)(L)}$.
The results follows from a comparison between these two direct sum decompositions.
\end{prop}

\begin{rmk}
Such an endofunctor $\sigma$ can be decomposed as a (directed) graph automorphism $\sigma_G$  and a functor $F$  on $\cat{Vect}_k$. If $F$ is covariant, then $\sigma_G$ preserves the directions. If $F$ is contravariant, then $\sigma_G$ reverse all the directions.
\end{rmk}

%\begin{rmk*}
%In another word, $\sigma$ is a natural transformation, if we view objects in $\cat{rep} Q$ as functors.
%\end{rmk*}

\subsection*{Operations induced by boundary compression}

\begin{defn}
Let $\ast$ denote a boundary compression method. This amounts to specifying the following functors\footnote{See Lemma 0 of the note \textit{2020-08-18(境界圧縮について)}} for each $I\in\mathcal{I}$:
\[
\opn{cmp}_I^*(-)\colon \cat{rep}\ Q \to \cat{rep}\ A_p.
\]
Here the positive integer $p$ is determined by $\ast$.
It is easy to verify that $\opn{cmp}_I^*$ is essentially surjective for each $I\in\mathcal{I}$.

We define the corresponding multiplicity:
\[
c^*_M(I) \coloneqq d_{\opn{cmp}_I^*(M)}\big(\opn{cmp}^*_I I\big)
\]

Let $\sigma$ be a functor as in Proposition $\ref{prop:endo}$. Furthermore, if it satisfies:
\begin{itemize}
    \item $\sigma$ is an automorphism on $\mathcal{I}$.
\end{itemize}

Then for each $I\in\mathcal{I}$, $\sigma$ and $*$ induces a new endofunctor $\sigma^*$ on $\cat{rep}\ A_p$:
\begin{equation}\label{eq:sigma-star}
    \sigma^*\big(N\big)=\sigma^*\big(\opn{cmp}^*_I(M)\big) \coloneqq \opn{cmp}^*_{\sigma(I)}(\sigma(M)).
\end{equation}
THIS IS NOT WELL-DEFINED, cause the boundary compression on $I$ and $\sigma(I)$ might not be compatible. (Even the $A_p$ types can be different).

Correct only if * defined on $I$ and $\sigma(I)$ are compatible.

Where we used the fact that $\opn{cmp}_I^*$ is essentially surjective, and we can verify that the choice of $M$ does not affect the result. 
%In fact, it suffices to verify it on $\mathcal{L}_{\cat{rep}\ A_p}$.

In particular, we can verify that $\sigma^*$ satisfies the conditions in the Proposition \ref{prop:endo}.
\end{defn}

\begin{lemma}
Let $*$ denote a boundary compression method and $\sigma$ be an endofunctor as specified in the definition above.
Then the $\delta^*$-multiplicity\footnote{See note \textit{2020-11-20(CL(3)の直既約分解)}} satisfies 
\[
\delta^*_{\sigma(M)}(I)=\delta^*_M\big(\tau(I)\big),
\qquad \forall\ M\in\cat{rep}\ Q
\]
\begin{proof}
It is NOT suffices to prove that ($\tau$ on the join of $S$)
\[
c^*_{\sigma(M)}(I)=c^*_M\big(\tau(I)\big),
\]
which amounts to showing that
\[
d_{\opn{cmp}_I^*\sigma(M)}\big(\opn{cmp}^*_I I\big)
=
d_{\opn{cmp}_{\tau(I)}^*M}\big(\opn{cmp}^*_{\tau(I)} {\tau(I)}\big).
\]
\end{proof}
Notice that 
\[
\begin{aligned}
d_{\opn{cmp}_I^*\sigma(M)}\big(\opn{cmp}^*_I I\big) &= d_{\sigma^*(\opn{cmp}_{\tau(I)}^*M)}\big(\opn{cmp}^*_I I\big)\\
&= d_{\opn{cmp}_{\tau(I)}^*M}\Big(\tau^*\big(\opn{cmp}^*_I I\big)\Big),
\end{aligned}
\]
which concludes the proof.
\end{lemma}

\begin{exa}\label{exa:sigma}
$\sigma$ on $\cat{CL}(n)$ for n = 2,3,4,5:
This functor can be described as:
\begin{enumerate}
    \item Apply the dual functor ($\Hom_k(-,k)$) on the diagram, then all arrows are reversed. Notice that now we are in the category $\cat{rep} \opn{CL(bbb)}$.
    \item Rotate the whole diagram by 180 degrees (a rotation functor).
\end{enumerate}
In this case the inverse of $\sigma$ is itself, and it satisfies all conditions needed.
\end{exa}

\begin{rmk}
If we notice that:
\begin{itemize}
    \item there exists a canonical isomorphism $V\cong V^*$ for finite dimensional vector spaces;
    \item taking the dual of a map amounts to take the transpose of its matrix representation.
    \item the rotation above can be decomposed as two reflections.
\end{itemize}
Then the following description might be more helpful when doing calculations. With a given $M\in \cat{rep}\ Q$, we apply the following operations in order
\begin{enumerate}
    \item reflects it along the horizontal middle line, and take each vertical map to its transposes (not commutative at this stage);
    \item reflects along the vertical middle line, with  each horizontal map taken to its transpose.
\end{enumerate}
\end{rmk}



\begin{exa}
See step 2 of \textit{2020-11-20(CL(3)の直既約分解)} for an illustration with the $\sigma$ defined above.
\end{exa}

==> legacy/__0099.tex <==
\section{On the computation of CL(4)}

\subsection{Continuation of the linear functions part}

\begin{itemize}
    \item $\mathcal{L}=\set{N_1,\cdots,N_{21},I_1,\cdots,I_{55}}$;
    \item $f_j(M)=c_M^*(I)$ for various combination of $I\in \mathcal{I}$ and $*$'s.
\end{itemize}
 have  and 

\begin{itemize}
    \item Some problems in both the code and the theoretical part.
    \item Equation \ref{eq:sigma-star} cannot be applied directly in general (Example, ss on 26 and zg on 49).
    \item Need to compute the c maps from $N_1$ to $N_21$
    \item We classify the intervals in order to find all possible new boundary compression methods.
\end{itemize}

\begin{enumerate}
    \item Zigzag-shaped: a total 40;
    \item Rectangle-shaped: 6 in total;
    \item Others: 9 in total: 26,27,29,34,35,36,39,45,49
\end{enumerate}

For each interval in the first and second category, there is only one boundary compression method (ss).

For each interval in the third category above, we can define two boundary compression methods: ss and zg.

For interval 36 and 29, we can further define another boundary compression method on them.

For interval 35, we can define another two boundary compression methods on it.

This amounts to a stacked matrix of rank 68, which is equal to the number of different boundary compression methods defined:
40+6+9*2+2+2=68


Outline of the paper
Title?
\begin{enumerate}
    \item Introduction
    \item Background
    \item Boundary compression, based on note 2020-08-06
    \item Indecomposable decomposition of CL(3), based on note
    \item Indecomposable decomposition of CL(4)
    \item Lesnick's theoory and Interval decomposition
    approximation
    \item numerical computation and examples
    \item CL(n) for $n\geq 5$
\end{enumerate}

\subsection{Results}
Statistics of boundary compression methods definable on intervals.

%footnote for compression method

\begin{minipage}[t]{\linewidth}


%\begin{table}
%\centering
\begin{tabular}{c|c|c|c}
%\hhline{*{4}{=}}
\hhline{*{4}{-}}
Category & Description & Number / Illustration & Compression method(s)\footnotemark\\\hhline{*{4}{=}}
    \multirow{2}{*}{Group 1}& 
    zigzag-shaped & 
    40 &
    \multirow{2}{*}{1} \\\hhline{~--~}
    & rectangle-shaped & 6 & \\ \hhline{----}
    \multirow{6}{*}{Group 2} & 
    $I_{26}$, $I_{49}$, $I_{34}$, $I_{45}$& 
    4 & 
    2 \\\hhline{~---}
    & $I_{27}$ &
    \scalebox{0.618}[0.618]{
    \begin{tikzcd}[ampersand replacement=\&,row sep=0.1em,column sep =0.2em]
\bullet \&\bullet \& \color{gray!50} \cdot \& \color{gray!50} \cdot \\
\bullet \&\bullet \&\bullet \&\bullet 
\end{tikzcd}}& 
    3  \\\hhline{~---}
    & $I_{39}$ &
    \scalebox{0.618}[0.618]{
    \begin{tikzcd}[ampersand replacement=\&,row sep=0.1em,column sep =0.2em]
\bullet \&\bullet \&\bullet \&\bullet \\
\color{gray!50} \cdot \&\color{gray!50} \cdot \&\bullet \&\bullet 
\end{tikzcd}}& 
    3  \\\hhline{~---}
        & $I_{29}$ &
    \scalebox{0.618}[0.618]{
    \begin{tikzcd}[ampersand replacement=\&,row sep=0.1em,column sep =0.2em]
\bullet \&\bullet \&\bullet \&\color{gray!50} \cdot \\
\bullet \&\bullet \&\bullet \&\bullet 
\end{tikzcd}}& 
    5   \\\hhline{~---}
        & $I_{36}$ &
    \scalebox{0.618}[0.618]{
    \begin{tikzcd}[ampersand replacement=\&,row sep=0.1em,column sep =0.2em]
\bullet \&\bullet  \&\bullet  \&\bullet  \\
\color{gray!50} \cdot \&\bullet  \&\bullet  \&\bullet  
\end{tikzcd}}& 
    5  \\\hhline{~---}
        & $I_{35}$ &
    \scalebox{0.618}[0.618]{
    \begin{tikzcd}[ampersand replacement=\&,row sep=0.1em,column sep =0.2em]
\bullet \&\bullet  \&\bullet \&\color{gray!50} \cdot \\
\color{gray!50} \cdot\&\bullet  \&\bullet  \&\bullet  
\end{tikzcd}}& 
    6   \\\hhline{*{4}{=}}
    Total & intervals of CL(4) & 55 & 76\\
    \hhline{*{4}{-}}
\end{tabular}
\captionof{table}{Caption}
\label{tab:my_label}
%\end{table}
\end{minipage}
\footnotetext{Number of independent boundary compression method(s) definable on each element in this group.}

\[
\begin{tikzcd}[row sep=0.4em,column sep = 0.1em]
\bullet &\cdot &\cdot &\cdot \\
\textcolor{gray}{\bullet} &\color{red} \cdot &\cdot &\cdot 
\end{tikzcd}
\]


\[
\scalebox{0.618}[0.618]{
    \begin{tikzcd}[ampersand replacement=\&,row sep=0.1em,column sep =0.2em]
1 \&1 \&1 \&1 \\
0 \&0 \&1 \&1 
\end{tikzcd}}
\]

==> legacy/cl4.tex <==
\subsection{Classification of tours}

some lemmas in 2020-08-18

to section 4
same as boundary compression to modules
 4. applications:
 cl 2,3,4
 
in-degree,out-degree,difference?

\begin{figure}[H]
\centering
\[
\begin{tikzcd}
\textcolor{red}{\overset{ss}{\bullet}}\arrow[r]&
\textcolor{blue}{\overset{cc}{\bullet}} \arrow[r] &
\circ \arrow[r]& 
\textcolor{red}{\overset{ss}{\bullet}} \\
&\textcolor{red}{\underset{ss}{\bullet}} \arrow[r]\arrow[u] &
\circ \arrow[r]\arrow[u]& 
\textcolor{blue}{\underset{cc}{\bullet}}\arrow[u] \\
\end{tikzcd}
\]
\caption{Illustration of ss-essential vertices and cc-essential vertices}
    \label{fig:cl_illu_1}
\end{figure}

\begin{figure}[H]
\centering
\[
\begin{tikzcd}
\textcolor{red}{\overset{ss}{\bullet}}\arrow[r]&
\textcolor{blue}{\overset{cc}{\bullet}} \arrow[r] &
\circ \arrow[r]& 
\textcolor{red}{\overset{ss}{\bullet}} \\
&\textcolor{red}{\underset{ss}{\bullet}} \arrow[r]\arrow[u] &
\circ \arrow[r]\arrow[u]& 
\textcolor{blue}{\underset{cc}{\bullet}}\arrow[u] \\
\end{tikzcd}
\]
\caption{Illustration of ss-essential vertices and cc-essential vertices}
    \label{fig:cl_illu_ss_cc}
\end{figure}
 
 
\[
\begin{tikzcd}
\textcolor{red}{\overset{ss}{\bullet}}\arrow[r]&
\textcolor{blue}{\overset{cc}{*}} \arrow[r] &
\circ \arrow[r]& 
\textcolor{red}{\overset{ss}{\bullet}} \\
&\textcolor{red}{\underset{ss}{\bullet}} \arrow[r]\arrow[u] &
\circ \arrow[r]\arrow[u]& 
\textcolor{blue}{\underset{cc}{*}}\arrow[u] \\
\end{tikzcd}
\]

\[
\begin{tikzcd}
\textcolor{red}{\overset{ss}{\bullet}}\arrow[r]&
\circ \arrow[r] &
\circ \arrow[r]& 
\textcolor{red}{\overset{ss}{\bullet}} \\
&\textcolor{red}{\underset{ss}{\bullet}} \arrow[r]\arrow[u] &
\circ \arrow[r]\arrow[u]& 
\circ\arrow[u] \\
\end{tikzcd}
\]

==> legacy/legacy_stability_sec5/0051-old-def.tex <==
\begin{defn}
Consider a $\cln$-shaped filtration simplicial complices as below:
%representation
\begin{equation}\label{eq:cln-filtration}
    \begin{aligned}
    \begin{tikzcd}
    Y_1\arrow[r]&Y_2\arrow[r]&\cdots\arrow[r]&Y_n\\
    X_1\arrow[r]\arrow[u]&X_2\arrow[r]\arrow[u]&\cdots\arrow[r]&X_n\arrow[u].
    \end{tikzcd}
    \end{aligned}
\end{equation}
Denote the filtration in the lower row as $X$, and the one in the upper row as $Y$. 
Notice that they are both $\mathbb{A}_n$-shaped filtrations. Compute the persistence diagram (after applying a specified homology functor at dimension $q$) of them and keep their respective interval information as
%\textcolor{red}{use symbol Imn ?}
\begin{itemize}
    \item $D_q(Y)=\Set{\big([b_j,d_j],m_j\big) | [b_j,d_j]\in \overline{\mathbb{R}}^2,\ m_j\in\mathbb{N},\ j\in J}$;
    \item $D_q(X)=\Set{\big([b_i,d_i],m_i\big) | [b_i,d_i]\in \overline{\mathbb{R}}^2,\ m_i\in\mathbb{N},\ i\in I}$.
\end{itemize}
Where each pair $[b_i,d_i]$ is distinct and $m_i$ records the multiplicity.
For each pair $([b_i,d_i],m_i)\in D_q(X)$ and $([b_j,d_j],m_j)\in D_q(Y)$ that satisfies:
\begin{enumerate}
    \item $b_i\leq d_j$ ;%(overlaps);
    \item $b_j\leq b_i$ and $d_j\leq d_i$ .%(together they form a staircase shape).
\end{enumerate}
Denote the interval subquiver consists of vertices located within the birth and death indices as $\mathbb{I}\big[\substack{b_j\ d_j\\ b_i\ d_i}\big]$:
\[
\begin{tikzcd}[column sep=small,row sep=small]
&\overset{b_j}{\bullet}\arrow[r]&\cdots\arrow[r]&\bullet\arrow[r]&\cdots\arrow[r]&\overset{d_j}{\bullet} \\
&&                               &\underset{b_i}{\bullet}\arrow[r]\arrow[u]&\cdots\arrow[r]&\bullet\arrow[u]\arrow[r]&\cdots\arrow[r]&\underset{d_i}{\bullet}
\end{tikzcd}.
\]
We use the interval approximation $l_{ji}\coloneqq \delta_M^\xi(V_{\mathbb{I}\big[\substack{b_j\ d_j\\ b_i\ d_i}\big]})$ 
to measure the persistence of the two features in the vertical direction. Here $\xi$ is a predetermined essential assignment and $M$ is the representation obtained from equation (\ref{eq:cln-filtration}).

A connected persistence diagram is a diagrammatic visualisation of the triplet $(D_q(Y),D_q(X),\set{l_{ji}}_{j\in J,i\in I})$ consists of the following three components:
\begin{itemize}
    \item $D_q(Y)$ visualised as an ordinary persistence diagram, fits into the upper left triangle region of the diagram;
    \item $D_q(X)$ fitted into the lower right triangle region of the diagram with the horizontal axis being death radius and vertical axis being birth radius. Compared with an ordinary persistence diagram, it is flipped along the diagonal line;
    \item for each non-zero $l_{ji}$, a line segment connecting the corresponding generators $(b_j,d_j)\in D_q(Y)$ and $(b_i,d_i)\in D_q(X)$.
\end{itemize}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.4\textwidth]{images/placeholder-image.jpg}
    \caption{Illustration of the structure of a connected persistence diagram}
    \label{fig:my_label}
\end{figure}
\end{defn}


\begin{itemize}
    \item For an interval $I$ in $\mathbb{I}_2$,
    set its multiplicity $m_I$ to be $\delta_M^\xi(V_I)$.
    % set its multiplicity $m_2^{(j)}$ to be $\delta_M^\xi(V_{[b^{(j)}_2,d^{(j)}_2]_2})$.
    Keep the birth-death coordinates and multiplicity obtained from all intervals in $\mathbb{I}_2$ as 
    $D_q^{\xi}(Y)=\Set{\big(I,m_I \big) | I\in \mathbb{I}_2 }$, 
    % $D_q^{\xi}(Y)=\Set{\big([b_2,d_2]_2,m_2^{(j)} \big) | j\in J }$, 
    it can be viewed as a persistence diagram.
    %%%%%%%%%
    \item For an interval $I$ in $\mathbb{I}_1$,
    set its multiplicity $m_I$ to be $\delta_M^\xi(V_I)$.
    The information from all intervals in $\mathbb{I}_1$ such obtained is denoted as $D_q^{\xi}(X)=\Set{\big(I,m_I \big) | I\in \mathbb{I}_1 }$.
    %%%%%%%%%
    \item For an interval $I$ in $\big(\mathbb{I}_{n,2}\big)_{\substack{2\\ 1}}$,
    let $m_I=\delta_M^\xi(V_I)$ measure the persistence of the two features in the vertical direction. 
    Keep the information as ${D_q^{\xi}(\substack{Y\\X})\coloneqq\Set{\big(I,m_I \big) | I\in \mathbb{I}_{\substack{2\\ 1}} }}$
\end{itemize}

==> legacy/legacy_stability_sec5/00540_stab.tex <==
% Tame: possible to parametrise
% wild: cannot be parameterised
% https://profs.sci.univr.it/~vitoria/visualintrotilting.pdf

% After defining connected persistence diagrams, we are immediately concerned with whether they have a stability theorem demonstrating their practical usefulness. 
% in light of the fact that interval-decomposability is not inherent in the definition of connected persistence diagrams.
A stability theorem is a crucial aspect of practical usefulness for any topological invariants.
While a stability result for general $\cln$ representations would be preferred, 
we lack the necessary techniques to handle such cases at this stage.
In this subsection, we provide a weaker version of the theorem that demonstrates the stability of connected persistence diagrams with respect to interval-decomposable representations. 
This result serves as a starting point and aims to motivate further research towards a general stability theorem.


\subsubsection{Interleaving Distance on Representations of Commutative Grids}

The usual shift functors employed in a stability theorem for infinite 2D commutative grids cannot be applied directly to our setting due to the restriction of two rows \cite{lesnick2015theory}.
To determine an appropriate interleaving distance for $\rep(\cln)$, we propose several families of endofunctors on commutative grids that generalize the shift functors.
Among those families, we select two that are suitable for the special two-layer structure of commutative ladders.
With these choices, we define an interleaving distance for $\rep\big(\cln\big)$ that allows for relaxed operations in the horizontal direction, but restricted freedom in the vertical direction.
We then define a distance between two connected persistence diagrams and demonstrate that 
it is stable with respect to the interleaving distance, following the logical structure of the proof in \cite{hiraoka2020algebraic}.

Throughout this subsection, the term ``distance" refers to a pseudometric.
% , and one-based indexing is adopted.

%slip functor?

\begin{defn}
Let $\vv{G}_{\infty,\infty}$ denote the infinite 2D equioriented commutative grid with integer coordinates. 
Consider the representation category $\rep(\vv{G}_{\infty,\infty})$.
% , whose underlying grid is $\mathbb{Z}\times \mathbb{Z}$.
A representation $M\in\rep(\Gpq)$ can be regarded as embedded in $\rep(\vv{G}_{\infty,\infty})$
aligned to the grid $\set{1,\cdots,p}\times\set{1,\cdots,q}$, and padded with zero-dimensional vector spaces around it.

We define two families of endo-functors. In both families, $c$ is a threshold value, and $s$ specifies the distance of translation.
\begin{enumerate}
    %horizontal
    \item 
    The \textit{horizontal dislocation functor $\mathcal{H}_c(s)$} is defined for $c\in \set{1,\cdots q}$ and $s\in \mathbb{Z}_{\geq 0}$ on a representation $M$ in the category $\rep(\vv{G}_{\infty,\infty})$. It shifts all vector spaces on or above the straight line $y=c$ leftwards by a unit $s$. 
    Specifically, for $(x,y)\in \mathbb{Z}\times\mathbb{Z}$, we have
    \[
    \begin{aligned}
    \mathcal{H}_c(s)\colon
    \rep(\Ginf)&\to \rep(\Ginf)\\
    M&\mapsto 
    \Biggl(
    (x,y)\mapsto \begin{cases}
    M_{(x+s,y)}& y\geq c\\
    M_{(x,y)}&y<c
    \end{cases}
    \Biggr)
    .
    \end{aligned}
    \]
    Morphisms between vector spaces are inherited from $M$.
    \textcolor{green}{this means that at the boundary line,....}
    \textcolor{red}{say that after the dislocation, it is still a representation of $\rep(\vv{G}_{\infty,\infty})$. (commutativity)}
    %vertical
    \item The \textit{vertical dislocation functors $\mathcal{V}_c(s)$} is defined for $c\in \set{1,\cdots,p}$ and $s\in \mathbb{Z}_{\geq 0}$ on a representation $M$ in the category $\rep(\vv{G}_{\infty,\infty})$.
    It shifts all vector spaces on or to the right of the straight line $x=c$ downwards by a unit $s$.
    Specifically, for $(x,y)\in \mathbb{Z}\times\mathbb{Z}$, we have
    \[
    \begin{aligned}
    \mathcal{V}_c(s)\colon
    \rep(\Ginf)&\to \rep(\Ginf)\\
    M&\mapsto 
    \Biggl(
    (x,y)\mapsto \begin{cases}
    M_{(x,y+s)}& x\geq c\\
    M_{(x,y)}&x<c
    \end{cases}
    \Biggr)
    .
    \end{aligned}
    \]
    Similarly, morphisms between vector spaces are inherited from $M$.
\end{enumerate}
The part that is moved is called the \textit{slipped region}, and the part whose associated spaces are fixed is called the \textit{unslipped region}. These names come from material science.
\end{defn}

\begin{rmk}
There is a natural transformation from the identity functor $\id$ to $\mathcal{H}_c(s)$ (\textit{resp.} $\mathcal{V}_c(s)$), where the map from $M_{(x,y)}$ to $\big(\mathcal{H}_c(s)(M)\big)_{(x,y)}$ (\textit{resp.} $\big(\mathcal{V}_c(s)(M)\big)_{(x,y)}$) is constructed from composition of linear maps within $M$ (which is well-defined by full commutativity). This map is called the \textit{transition morphism}.
\end{rmk}

% we can also work with $\vv{G}_{+\infty,+\infty}$ to avoid the technical details of truncation of representations and padding zero-dimensional vector spaces. In practice, it suffices to find a large enough grid to fit the original representation.
\begin{figure}[H]
    \centering
    \begin{subfigure}{0.33\textwidth}
    \includegraphics[width=\linewidth]{images/horizontal_dislocation_functor.pdf}
    \caption{}
    \end{subfigure}
    % \hspace*{\fill}
    \hspace{.2\linewidth} 
    \begin{subfigure}{0.33\textwidth}
    \includegraphics[width=\linewidth]{images/vertical_dislocation_functor.pdf}
    \caption{}
    \end{subfigure}
    \caption{Illustration of the horizontal dislocation functor $\mathcal{H}_c(s)$ and the vertical dislocation functor $\mathcal{V}_c(s)$ with their corresponding slipped regions. The colored areas represent where vector spaces will be translated by $s$ units to the indicated direction.}
\label{fig:dislocation_functors}
\end{figure}

\begin{rmk}
We can express the shift functor $\mathcal{T}(a,b)$, which maps $(x,y)$ to $M_{(x+a,y+b)}$ when applied to $M$, as the composition  $\mathcal{H}_{-\infty}(a)\circ\mathcal{V}_{-\infty}(b)$.
\end{rmk}

\begin{rmk}
In the definition above, we used vertical and horizontal lines as boundaries.
However, a more general family of straight lines can be used to define a dislocation functor. 
These functors can be further generalized to settings with more parameters, where the boundary line becomes a hyperplane.
We note that the counterparts of these functors can also be defined in the continuous poset setting $\mathbb{R}^2$.
\end{rmk}


\begin{exa}
In Figure \ref{fig:tour_types}, we presented several ways to define zigzag courses from a commutative ladder.
We note that horizontal and vertical dislocation functors can be used to transform (non-zigzag) representations of $\Gpq$ to zigzag representations in a functorial manner. Below, we provide two examples to illustrate this idea.

The figures below depict two distinct yet functorial approaches to transforming a representation of $\vv{G}_{3,2}$ into a zigzag representation.
Note that we begin with the initial position of $u$ at coordinate $(1,1)$.
\begin{itemize}
    \item $\mathcal{V}_2(1)\circ \mathcal{H}_2(1)$:
\[
\begin{tikzcd}[column sep=normal, row sep=normal]
x \arrow[r, "\gamma"] & y \arrow[r, "\delta"] & z \\
u\arrow[u, "\epsilon"] \arrow[r, "\alpha"'] & v \arrow[r, "\beta"']  \arrow[u, "\zeta"] & w \arrow[u, "\eta"]
\end{tikzcd}
\xRightarrow{\mathcal{H}_2(1)}
% second step
\begin{tikzcd}[column sep=normal, row sep=normal]
x\arrow[r, "\gamma"] & y \arrow[r, "\delta"] & z & \\
& u \arrow[u, "\gamma\circ\epsilon"] \arrow[r, "\alpha"'] & v \arrow[r, "\beta"']  \arrow[u, "\delta\circ\zeta"'] & w
\end{tikzcd}
\xRightarrow{\mathcal{V}_2(1)}
% third step
\begin{tikzcd}[column sep=normal, row sep=normal]
x\arrow[r, "\gamma"] & y & & \\
& u \arrow[u, "\gamma\circ\epsilon"] \arrow[r, "\delta\circ\gamma\circ\epsilon"'] & z & \\
&& v \arrow[r, "\beta"']  \arrow[u, "\delta\circ\zeta"'] & w
\end{tikzcd}
\]
\item $\mathcal{H}_2(2)$:
\[
\begin{tikzcd}[column sep=normal, row sep=normal]
x \arrow[r, "\gamma"] & y \arrow[r, "\delta"] & z \\
u\arrow[u, "\epsilon"] \arrow[r, "\alpha"'] & v \arrow[r, "\beta"']  \arrow[u, "\zeta"] & w \arrow[u, "\eta"]
\end{tikzcd}
\xRightarrow{\mathcal{H}_2(2)}
% second step
\begin{tikzcd}[column sep=normal, row sep=normal]
x\arrow[r, "\gamma"] & y \arrow[r, "\delta"] & z && \\
&& u \arrow[u, "\delta\circ\gamma\circ\epsilon"] \arrow[r, "\alpha"'] & v \arrow[r, "\beta"']  & w
\end{tikzcd}
\]
\end{itemize}
%%%%%%%%%%%%
The different ways of expressing a composite map are equivalent by commutative relations.
\end{exa}

\begin{rmk}
It is easy to verify that horizontal dislocation functors and vertical dislocation functors commute within a same family,
but are not commutative when mixed together.
Due to this property and the two-layer structure of $\cln\subseteq\clinf\coloneqq\vv{G}_{\infty,2}$, 
we will use the subfamilies $\mathcal{H}_1(s)$ and $\mathcal{H}_2(s')$ for $s,s'\in \set{1,\cdots,n}$ 
in our stability theorem for connected persistence diagrams.
\end{rmk}

\begin{defn}[Interleaving Distance]\label{defn:interleaving-distance}
Let $\vdel\coloneqq (\delta_1,\delta_2)$ be a tuple in $\mathbb{Z}^2_{\geq 0}$.
Define the associated dislocation functor $\mathcal{T}_{\vdel}$ 
%T for 転移
as a composition of two horizontal dislocation functors (notice that they are commutative):
\[
\mathcal{T}_{\vdel}\coloneqq \mathcal{H}_2(\delta_2)\circ\mathcal{H}_1(\delta_1).
\]
% and consistency with the notation used in stability theorems,
To simplify the notation, 
we will use $M(\vdel)$ to represent the image of $M$ under the dislocation functor $\mathcal{T}_{\vdel}$.
Two representation $M,N\in\rep(\cln)\subseteq\rep(\clinf)$ are said to be \textit{$\vdel$-interleaved}
if there exists a pair of morphisms 
$M\xrightarrow{f}N(\vdel)$ 
and 
$N\xrightarrow{g}M(\vdel)$ (both called $\vec{\delta}$-interleaving morphisms) such that
the natural morphism from $M$ to $M(2\vdel)$ factors through $N(\vdel)$
and the natural morphism from $N$ to $N(2\vdel)$ factors through $M(\vdel)$:
\begin{equation}
\begin{minipage}{0.45\textwidth}
\centering
    \begin{tikzcd}[column sep=small]
    M\arrow[rr]\arrow[rd,"f"']&&M(2\vdel)\\
    &N(\vdel)\arrow[ru,"g(\vdel)"']\arrow[ru,bend left=45,near start,phantom,"\circlearrowleft"]&
    \end{tikzcd},
\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}
\centering
    \begin{tikzcd}[column sep=small]
    N\arrow[rr]\arrow[rd,"g"']&&N(2\vdel)\\
    &M(\vdel)\arrow[ru,"f(\vdel)"']\arrow[ru,bend left=45,near start,phantom,"\circlearrowleft"]&
    \end{tikzcd}.
\end{minipage}
\end{equation}
The interleaving distance between $M$ and $N$ is defined to be
% could 2\cdot\norm{\vdel}_{\infty} be used instead?
\[
d_I(M,N)
=\inf\set{\norm{\vdel}_{1}|
\text{
$M$ and $N$ are $\vdel$-interleaved
}
}.
\]
\end{defn}

\begin{rmk}
Let $M$ be a representation in $\rep(\cln)\subseteq\rep(\clinf)$.
We call it \textit{$\vec{\delta}$-trivial} if it is $\vec{\delta}$-interleaved with the zero representation $\mathbf{0}$.
Assuming that $n$ is even for simplicity,
the $M\big((n,0)\big)_{(x,y)}=M_{x+n,y+n}$.
Thus, the morphism $M\to M\big((n,0)\big)$ is a zero morphism,
which factors through $\mathbf{0}\big((n/2,0)\big)$, 
so we conclude that $M$ is ${(n/2,0)}$-trivial and $d_I(M,\mathbf{0})\leq n $. 
For any three representations $L,M,N\in \rep(\cln)\subseteq\rep(\clinf)$, if $L$ and $M$ are $\vec{\gamma}$-interleaved
and $M$ and $N$ are $\vec{\delta}$-interleaved, 
then we have that $L$ and $N$ are $(\vec{\gamma}+\vec{\delta})$-interleaved.
Therefore, the interleaving distance is defined for representations in $\rep(\cln)\subset\rep(\clinf)$, and for any two such representations $M,N$,
we have $d_I(M,N)\leq 2 n$.
\end{rmk}

==> legacy/legacy_stability_sec5/00540_stab_original.tex <==
% Tame: possible to parametrise
% wild: cannot be parameterised
% https://profs.sci.univr.it/~vitoria/visualintrotilting.pdf

Following the definition of connected persistence diagrams, the immediate next thing we care about is whether there is a stability theorem for it, which justifies its usage in practical problems.

However, the usual translation functors used in a stability theorem in an infinite 2D commutative grid are not applicable to our settings here.
Therefore, we propose several families of endofunctors on commutative grids, show that it generalizes the translation functors.

We will pick out two families of functors that fits into the special two-layer structure of commutative ladders. 
Using that choice, an interleaving distance for $\rep(\cln)$ can be defined, it is equipped with relaxed operations in the horizontal directions but restricted freedom in the vertical direction. We then define a distance for two cPDs, and show that this distance is stable with respect to the interleaving distance. We follow the logical structure of the proof of the algebraic stability theorem in \cite{hiraoka2020algebraic}. In this part, distance refers to a pseudometric. We will use one-based indexing throughout this subsection.


%slip functor?
\begin{defn}
Consider the representation category $\rep(\vv{G}_{\infty,\infty})$, whose underlying grid is $\mathbb{Z}\times \mathbb{Z}$.
A representation $M\in\rep(\Gpq)$ can be regarded as embedded in $\rep(\vv{G}_{\infty,\infty})$
to the grid $\set{1,\cdots,p}\times\set{1,\cdots,q}$, padded with zero-dimensional vector spaces around.
We define the following two families of endo-functors:
% where an index that goes beyond the range maps to zero.
\begin{enumerate}
    %vertical
    \item \textit{vertical dislocation functors $\mathcal{V}_c(s)$}, where $c\in \set{1,\cdots,p}$ and $s\in \mathbb{Z}_{\geq 0}$.
    Applied on a representation $M$, this functor shifts all vector spaces on or above the line $x=c$ by a unit $s$, that is:
    \[
    \begin{aligned}
    \mathcal{V}_c(s)\colon
    \rep(\Ginf)&\to \rep(\Ginf)\\
    M&\mapsto 
    \Biggl(
    (x,y)\mapsto \begin{cases}
    M_{(x,y+s)}& y\geq c\\
    M_{(x,y)}&y<c
    \end{cases}
    \Biggr)
    .
    \end{aligned}
    \]
    Morphisms between vector spaces are inherited from $M$.
    %horizontal
    \item \textit{horizontal dislocation functor $\mathcal{H}_c(s)$}, where $c\in \set{1,\cdots q}$ and $s\in \mathbb{Z}_{\geq 0}$. 
    Applied on a representation $M$, this functor shifts all vector spaces on or above the line $y=c$ by a unit $s$, that is:
    \[
    \begin{aligned}
    \mathcal{H}_c(s)\colon
    \rep(\Ginf)&\to \rep(\Ginf)\\
    M&\mapsto 
    \Biggl(
    (x,y)\mapsto \begin{cases}
    M_{(x+s,y)}& x\geq c\\
    M_{(x,y)}&x<c
    \end{cases}
    \Biggr)
    .
    \end{aligned}
    \]
    Similarly, morphisms between vector spaces are inherited from $M$.
\end{enumerate}
We will call the part that is moved the slipped region, the part with associated spaces being fixed the unslipped region. These namings come from materials science.
\end{defn}

\begin{rmk}
There is a natural transformation from the identity functor $\id$ to $\mathcal{V}_c(s)$ (\textit{resp.} $\mathcal{H}_c(s)$), where the map from $M_{(x,y)}$ to $\big(\mathcal{V}_c(s)(M)\big)_{(x,y)}$ (\textit{resp.} $\big(\mathcal{H}_c(s)(M)\big)_{(x,y)}$) is defined in the obvious way. This map is called the \textit{transition morphism}.
\end{rmk}

% we can also work with $\vv{G}_{+\infty,+\infty}$ to avoid the technical details of truncation of representations and padding zero-dimensional vector spaces. In practice, it suffices to find a large enough grid to fit the original representation.
\begin{exa}
Illustration. To be updated
\end{exa}
\begin{rmk}
Existing stability theorems in multi-parameter persistent homology have been using translations.
It is easy to see that the translation functor $\mathcal{T}(a,b)$, which maps $(x,y)$ to $M_{(x+a,y+b)}$ when applied on $M$,
can be expressed as a composition $\mathcal{H}_{-\infty}(a)\circ\mathcal{V}_{-\infty}(b)$.
More generally, we can also define a dislocation functor with the boundary line being $y=kx+b$.
These functors can also be defined when using the continuous poset settings $\mathbb{R}^2$. In particular, for more parameters, the boundary line becomes a hyperplane.
\end{rmk}

\begin{rmk}
It is easy to see that horizontal dislocation functors and vertical dislocation functors are commutative on their own 
but are not commutative when getting mixed.
Due to this reason and the two-layer structure of $\cln\subseteq\clinf\coloneqq\vv{G}_{\infty,2}$, 
we will use the subfamilies $\mathcal{H}_0(s)$ and $\mathcal{H}_1(s')$ with $s,s'\in \set{0,\cdots,n-1}$ in our stability theorem for cPDs.
\end{rmk}

\begin{defn}[interleaving distance]
Let $\vdel\coloneqq (\delta_1,\delta_2)$ be a tuple in $\mathbb{Z}^2_{\geq 0}$.
Define the associated dislocation functor $\Delta_{\veps}$ as a composition of two horizontal dislocation functors (notice that they are commutative):
\[
\mathcal{D}_{\vdel}\coloneqq \mathcal{H}_2(\delta_2)\circ\mathcal{H}_1(\delta_1).
\]
For simplicity and following the convention of symbols used in stability theorems,
we denote ${M(\vdel)\coloneqq \mathcal{D}_{\vdel}(M)}$.
Two representation $M,N\in\rep(\cln)\subseteq\rep(\clinf)$ are said to be $\vdel$-interleaved 
if there exists a pair of morphisms 
$M\xrightarrow{f}N(\vdel)$ 
and 
$N\xrightarrow{g}M(\vdel)$ (both are called ($\vec{\delta}$-)interleaving morphisms) such that
the natural map from $M$ to $M(2\vdel)$ factors through $N(\vdel)$,
and the natural map from $N$ to $N(2\vdel)$ factors through $M(\vdel)$:
% That is, the following two diagrams each commutes:
% \begin{minipage}{.45\linewidth}
\begin{equation}
\begin{minipage}{0.45\textwidth}
\centering
    \begin{tikzcd}[column sep=small]
    M\arrow[rr]\arrow[rd,"f"']&&M(2\vdel)\\
    &N(\vdel)\arrow[ru,"g(\vdel)"']\arrow[ru,bend left=45,near start,phantom,"\circlearrowleft"]&
    \end{tikzcd},
\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}
\centering
    \begin{tikzcd}[column sep=small]
    N\arrow[rr]\arrow[rd,"g"']&&N(2\vdel)\\
    &M(\vdel)\arrow[ru,"f(\vdel)"']\arrow[ru,bend left=45,near start,phantom,"\circlearrowleft"]&
    \end{tikzcd}.
\end{minipage}
\end{equation}
The interleaving distance between $M$ and $N$ is defined to be
\[
d_I(M,N)
=\inf\set{\norm{\vdel}_{\infty}|
\text{
$M$ and $N$ are $\vdel$-interleaved
}
}.
\]
\end{defn}
\begin{rmk}
We say a representation $M$ is $\vec{\delta}$-trivial if it is $\vec{\delta}$-interleaved with the zero representation.
Assuming $n$ is an even number without loss of generality.
If $M\in\rep(\cln)\subseteq\rep(\clinf)$, 
then $M\to M\big((n,0)\big)$ is a zero morphism. 
As a result, $M$ is ${(n/2,0)}$-trivial and $d_I(M,\mathbf{0})\leq n $. 
If $L,M,N$ are all representations of $\rep(\cln)\subseteq\rep(\clinf)$, with $L$ and $M$ being $\vec{\gamma}$-interleaved, 
$M$ and $N$ being $\vec{\delta}$-interleaved, then it is easy to see that $L$ and $N$ are $(\vec{\gamma}+\vec{\delta})$-interleaved.
Therefore, the interleaving distance is defined on $\rep(\cln)\subset\rep(\clinf)$, and for any two representations $M,N$ in that category, $d_I(M,N)\leq 2 n$.

\end{rmk}
In contrast to a persistence diagram from one-parameter persistent homology, a connected persistence diagram contains many components that do not appear to be comparable at first sight. In particular, the multiplicity of an element in it can be negative.
These are all obstacles to defining a bottleneck distance on connected persistence diagrams directly.
To address these problems, we first disassemble elements in a connected persistence diagram into several sets, then define a pseudo-distance on connected persistence diagrams via finding a matching between those sets respectively.

\begin{defn}
Let $\cPD\coloneqq \Big(D_q^{\xi}(Y),D_q^{\xi}(X),D_q^{\xi}(\substack{Y\\X})\Big)$ be a connected persistence diagram.
The \textit{unpacking function} $\mu$ maps a connected persistence diagram to a tuple of four multisets, following the steps below:
\begin{enumerate}
    \item Construct the following three multisets:
    \begin{itemize}
        \item $U$: upper horizontal persistence;
        \item $L$: lower horizontal persistence;
        \item $V$: width of the vertical persistence.
    \end{itemize}
    \item Initially, add all elements in $D_q^{\xi}(Y)$ to $U$ and all elements in $D_q^{\xi}(X)$ to $L$. Elements in them are guaranteed to have positive multiplicities.
    \item For each $\big([b_1,d_1]_1\sqcup[b_2,d_2]_2,m\big)\in D_q^{\xi}(\substack{Y\\X})\Big)$, 
    %add $\big([b_2,d_2]_2,m\big)$ to $U$,
    %$\big([b_1,d_1]_1,m\big)$ to $L$,
    %and $\big([b_1,d_2]_2\sqcup[b_1,d_2]_1,m\big)$ to $V$. 
    add $\big([b_1,d_2]_1\sqcup[b_1,d_2]_2,m\big)$ to $V$. 
    \item %Separate elements in the three multisets according to the positivity of their multiplicity. Write the result as
    Separate elements in $V$ according to the positivity of their multiplicities. Write the set as a disjoint union:
    \begin{itemize}
        %\item $U=U^+\sqcup U^-$;
        %\item $L=L^+\sqcup L^-$;
        \item $V=V^+\sqcup V^-$.
    \end{itemize}
    \item Notice that an element $[b_1,d_2]_1\sqcup[b_1,d_2]_2$ in $V$ is guaranteed to have a rectangle shape, so it suffices to remove the redundant symbols and keep it as $\big([b_1,d_2],m)$, with the subscript ignored. We also ignore the subscripts of elements in $U$ and $L$ for simplicity.
    \item Finally, $\mu(\cPD)$ is a tuple $\big(U,L,V^+,V^-\big)$, 
    and an element in any of the sets can be written as $([b,d],m)$.
    For simplicity, we further remove all redundant brackets and 
    denote elements in form of $\abte{b}{d}{m}$.
    % and an element in any of the set can be written as $([b,d],m)$.
    % $\big(U^\pm,L^\pm,V^\pm\big)\coloneqq $
    % $[b,d]_{\square}$
\end{enumerate}
% It is easy to see that with the six multisets given above,
% a \textit{packing function} $\nu$ can be defined to retrieve original elements $\cPD$ by reconstructing  elements in $V$ first.
% No, it is not
% pack/unpack
% disassembly map
% assembly map
% uncouple/unpack
% cPD to two horizontal/vertical parts,
% further separated by positivity.
\end{defn}

We are going to vectorize several operations in the one-parameter persistent homology case to define their counterparts in $\mu(\cPD)$.

\begin{defn}
Let $\cPD$ be a connected persistence diagram,
$b$ and $d$ be two integers, $\delta$ be a non-negative integer.
For operations $\square\in\set{\delta,[-,d],[b,-]}$, we define
\[
% \mu(\cPD)_{\square}=\big(U^+_\square,U^-_\square,L^+_\square,L^-_\square,V^+_\square,V^-_\square\big).
\mu(\cPD)_{\square}=\big(U_\square,L_\square,V^+_\square,V^-_\square\big).
\]
For $\Lambda\in \set{U,L,V^\pm}$,
\begin{itemize}
    % \item $\Lambda_\delta\coloneqq \set{([b,d],m)\in\Lambda| d-b\geq \delta}$;
    \item $\Lambda_\delta\coloneqq \set{(\abte{b}{d}{m}\in\Lambda| d-b\geq \delta}$;
    % \item $\Lambda_\delta$ consists of elements $[b,d]\in\Lambda$ satisfying $d-b\geq \delta$;
    \item $\Lambda_{[-,d]}\coloneqq \set{\abte{u}{v}{m}\in\Lambda|v=d}$;
    \item $\Lambda_{[b,-]}\coloneqq \set{(\abte{u}{v}{m}\in\Lambda|u=b}$.
\end{itemize}
We will define an ordering on each of these multisets which puts important features first.
Equip $\Lambda_{[-,d]}$ with the following lexicographical order
induced by reverse inclusion relations on the birth-death pair and absolute values on the multiplicities:
\begin{itemize}
    % \item $([u,d],m)<([u',d],m')$ if and only if $u<u'$, or $u=u'$ and $|m|>|m'|$.
    \item $\abte{u}{d}{m}<\abte{u'}{d}{m'}$ if and only if $u<u'$, or $u=u'$ and $|m|>|m'|$.
\end{itemize}
Equip $\Lambda_{[b,-]}$ with the following lexicographical order:
\begin{itemize}
    % \item $([b,v],m)<([b,v'],m')$ if and only if $v'<v$, or $v=v'$ and $|m|>|m'|$.
    \item $\abte{b}{v}{m}<\abte{b}{v'}{m'}$ if and only if $v'<v$, or $v=v'$ and $|m|>|m'|$.
\end{itemize}
\end{defn}

\begin{rmk}    
It is easy to see that for $\Lambda=U, L$, the order of elements in $\Lambda_{[b,-]}$ and $\Lambda_{[-,d]}$ is not affected by $m$, 
as each $[b',d']$ pair is unique. However, this statement is not true for $\Lambda=V^\pm$. For example, both $([5,10]_1\sqcup [1,7]_2],1)$ and $[5,8]_1\sqcup [4,7]_2,1)$ contribute $([5,7],1)=\abte{5}{7}{1}$ to set $V^+$. 
% To simplify the notations and emphasize the totally ordered set structures, elements in $\Lambda_{[b,-]}$ and $\Lambda_{[-,d]}$ for $\Lambda\in\set{U,L,V^\pm}$ will be denoted as $\abte{b'}{d'}{m'}$, removing the square brackets. 
% As only the ordering is important instead of $m$'s value, if $m$ is superfluous in determining the ordering, as $\iprod{b}{d}$.
%??? add the sentence above ???
\end{rmk}

The unpacking function will help us to define a distance on the set of connected persistence diagrams.
Recall that a matching $\sigma$ between two sets $A$ and $B$, denoted as $\sigma\colon A\centernot\rightarrow B$, is a bijection between $A'\subseteq A$ and $B'\subseteq B$.
We denote $\Coim\sigma\coloneqq A'$ and $\Im\sigma\coloneqq B'$. If $\vv{\sigma}$ is a tuple of matchings, $\Coim\vv{\sigma}$ or $\Im\vv{\sigma}$ denote a tuple of sets where the operation is applied element-wisely.
% We define a matching $\vv{\sigma}$ between two tuples of multisets 
% $(S_i)_{i\in I}$ and $(T_i)_{i\in I}$
% to be a tuple of matchings $(\sigma_i)_{i\in I}$,
% where each $\sigma_i$ is a matching between $S_i$ and $T_i$.
\begin{defn}
Let $\cPD$ and $\cPD'$ be two connected persistence diagrams.
A $\delta$-matching between connected persistence diagrams $\cPD$ and $\cPD'$ 
is a tuple of matchings 
$\vv{\sigma}=
\big(
\sigma_{U},
\sigma_{L},
\sigma_{V^+},
\sigma_{V^-}
\big)$ 
between elements of $\mu(\cPD)$ and $\mu(\cPD')$
such that 
\[
\mu(\cPD)_{2\delta}\subseteq \Coim\vv{\sigma}
\qquad
\mu(\cPD')_{2\delta}\subseteq \Im\vv{\sigma}.
\]
The inclusions are meant to be evaluated element-wisely.
In addition, for all $\sigma_\square(\abte{b}{d}{m})=\abte{b'}{d'}{m'}$, we require that
\[
b'-\delta\leq b\leq d\leq d'+\delta,
\qquad
b-\delta\leq b'\leq d'\leq d+\delta.
\]
Two connected persistence diagrams are said to be 
\textit{$\delta$-matched} if there exists a $\delta$-matching 
between them.
\end{defn}

\begin{defn}
Let $\cPD$ and $\cPD'$ be two connected persistence diagrams.
The \textit{bottleneck distance} between $\cPD$ and $\cPD'$ 
is defined as 
\[
d_B(\cPD,\cPD')\coloneqq 
\inf\set{\delta\in \mathbb{Z}_{\geq 0}|
\text{
$\cPD$ and $\cPD'$ are $\delta$-matched}
}.
\]
\end{defn}

\begin{prop}
The bottleneck distance defined above is a pseudometric on the set of connected persistence diagrams.
\begin{proof}
    The only property that is not immediately obvious is the triangle inequality.
    Let $\vv{\sigma_1}$ be a $\delta_1$-matching between $\cPD$ and $\cPD'$, 
    $\vv{\sigma_2}$ be a $\delta_2$-matching between $\cPD'$ and $\cPD''$.
    Then it can be easily verified that the element-wise composition of the two matchings 
    is a $(\delta_1+\delta_2)$-matching between $\cPD$ and $\cPD''$, from which the triangle inequality follows.
\end{proof}
\end{prop}

We are going to prove that a morphism $f\colon M\to N$ 
induces a matching between the corresponding connected persistence diagrams. 
%canonical matching
If $S=\set{s_i|i=1,\cdots,|S|}$ and $T=\set{t_i|i=1,\cdots,|T|}$ are two finite totally ordered sets with partial orders both inferred from the subscript as a poset in $\mathbb{N}$, then a \textit{canonical matching} $\sigma\colon S\centernot\rightarrow T$ is defined by $\sigma(s_i)=t_i$ for $i=1,\cdots,\min\set{s,t}$, from which we have $\Im\sigma =S$ or $\Coim\sigma=T$.

This concept can be vectorized as below.
Let
\[
\vv{S}=(S^1,\cdots,S^m)\qquad
\vv{T}=(T^1,\cdots,T^m)
\]
be two tuples of finite totally ordered sets where $S^i=\set{s^i_j|j=1,\cdots,|S^i|}$ and $T^i=\set{t^i_j|j=1,\cdots,|T^i|}$.
Then a canonical matching $\vv{\sigma}\colon \vv{S}\centernot\rightarrow\vv{T}$ is a tuple of canonical matchings $(\sigma^1,\cdots,\sigma^m)$ such that each $\sigma^i$ is a canonical matching between $S^i$ and $T^i$.

\begin{defn}
Let $f\colon M\to N$ be a morphism in $\rep(\cln)$.
The induced matching 
\[
\mu(f)\colon \mu\big(\cPD(M)\big) \centernot\rightarrow \mu\big(\cPD(N)\big)
\]
\begin{enumerate}
    \item If $f$ is injective, $\mu(f)$ is the tuple of canonical matching from 
    $\mu\big(\cPD(M)\big)_{[-,d]}$
    to
    $\mu\big(\cPD(N)\big)_{[-,d]}$.
    \item If $f$ is subjective, $\mu(f)$ is the tuple of canonical matching from 
    $\mu\big(\cPD(M)\big)_{[b,-]}$
    to
    $\mu\big(\cPD(N)\big)_{[b,-]}$.
    \item In the general case, decompose $f$ as the composition of the following two maps:
    \[
        M\xrightarrow{\pi}\Im f\xrightarrow{\iota}N,
    \]
    where $\pi$ is surjective and $\iota$ is injective.
    Then $\mu(f)$ is defined to be $\mu(\iota)\circ\mu(\pi)$.
\end{enumerate}
\end{defn}


% Four ss-vertices lemma
\begin{lemma}\label{lemma:cPD-four-ss-vertices}
Let $M$ be a representation of $\cln\subseteq\clinf$ and $\vec{\delta}=(\delta_1,\delta_2)\in \mathbb{Z}^2_{\geq 0}$.
Denote $\cPD(M)$ as $\Big(D_q^{\xi}(Y),D_q^{\xi}(X),D_q^{\xi}(\substack{Y\\X})\Big)$
and
\[
\mu\Big(\cPD\big(M(\vec{\delta})\big)\Big)=\big(U(\vec{\delta}),L(\vec{\delta}),V^+(\vec{\delta}),V^-(\vec{\delta})\big)
\qquad \mbox{and}
\qquad
\mu\big(\cPD(M) \big)=\big(U,L,V^+,V^-\big).
\]
If each element $\big([b_1,d_1]_1\sqcup[b_2,d_2]_2,m\big)$ in $D_q^{\xi}(\substack{Y\\X})$ satisfies the following condition:
\[
b_1\neq b_2\quad \mbox{and}\quad d_1\neq d_2,
\]
then exists a $\vec{\delta}$-matching 
\[
r_M^{\vec{\delta}}\colon \mu\big(\cPD(M(\vec{\delta})) \big)
\centernot\rightarrow
\mu\big(\cPD(M) \big)
\]
abiding by the following rules:
\begin{itemize}
    \item $r_M^{\vec{\delta}}(\abte{b}{d}{m})=\abte{b+\delta_1+\delta_2}{d+\delta_1+\delta_2}{m}$ for elements in $U(\vec{\delta})$;
    \item $r_M^{\vec{\delta}}(\abte{b}{d}{m})=\abte{b+\delta_1}{d+\delta_1}{m}$ for elements in $L(\vec{\delta})$;
    \item $r_M^{\vec{\delta}}(\abte{b}{d}{m})=\abte{b+\delta_1}{d+\delta_1+\delta_2}{m}$ for elements in $V^\pm(\vec{\delta})$.
\end{itemize}
\begin{proof}
For $U(\vdel)$ and $L(\vdel)$ bijective.

For $V^\pm(\vdel)$, 
dissociated into two parts
remain associated via maps
bijective on intervals that are not dissociated, m stays the same
For intervals that are dissociated, $d-b\leq \delta_2$
\end{proof}
\end{lemma}


\begin{thm}[Induced matching theorem]
Let $f\colon M\to N$ be a morphism in $\rep(\cln)\subseteq\rep(\clinf)$, $\vec{\delta}$ be a tuple in $\mathbb{Z}^2_{\geq 0}$
where both $M$ and $N$ satisfy the condition in lemma \ref{lemma:cPD-four-ss-vertices}.
Assume that $\Ker f$ and $\Coker f$ are $2\vec{\delta}$-trivial.
Then we have a $\vec{\delta}$-matching
\[
\mu(f)\circ r_M^{\vec{\delta}}
\colon
\mu\Big(\cPD\big(M(\vec{\delta})\big)\Big)
\centernot\rightarrow
\mu(\big(\cPD(N)\big).
\]
\begin{proof}
\end{proof}
\end{thm}

\begin{prop}
If $M$ and $N$ are $\vdel$-interleaved with $f\colon M\to N(\vdel)$
being one interleaving morphism, then $\Ker f$ and $\Coker f$ are $2\vdel$-trivial.
\begin{proof}
\end{proof}
\end{prop}

\begin{thm}[Algebraic stability theorem]
Let $M$,$N$ be representations of $\Gpq$. Then
\[
d_B\big(\cPD(M),\cPD(N)\big)\leq 
d_I(M,N).
\]
\begin{proof}
\end{proof}
\end{thm}

% \begin{itemize}
%     \item Commutative ladder module $\rep(\cln)$ $\Rightarrow$
%     \item $\xi$-compressed multiplicities $\Rightarrow$
%     \item connected persistence diagrams
% \end{itemize}
% \vspace{10pt}
% Need to define the following two distances (pseudo-metric):
% \begin{itemize}
%     \item interleaving distance on $\rep(\cln)$
%     \item bottleneck distance on cPDs.
% \end{itemize}
% \vspace{10pt}
% Using the language of \textit{Theory of interleavings on categories with a flow} (see Definition 2.1 and Definition 3.1)

% \begin{defn}
% Settings
% \begin{itemize}
%     \item $\mathcal{P}\coloneqq \mathbb{R}\times \mathbb{F}_2$
%     \item $\mathcal{D}=\cat{Vect}_\Bbbk$
% \end{itemize}
% A commutative ladder module is a function $M\in \mathcal{D}^{\mathcal{P}}$ (or $\rep_{\mathbb{k}}(\mathcal{P})$)
% such that for any $(1,a),(1,b),(0,a),(0,b)$ with $a<b$, the corresponding square commutes.
% \vspace{10pt}
% We can define two kinds of flows on $\mathcal{P}$ (\textit{i.e.}, two families of endofunctors on $\mathcal{P}$.
% Let $\varepsilon\in [0,\infty)$
% \begin{enumerate}
%     \item overall shift functor $\mathcal{T}_{\varepsilon}$;
%     \item upper dislocation functor $\mathcal{U}_{\varepsilon}$;
%     %\item lower dislocation functor $\mathcal{L}_{\varepsilon}$; not a poset morphism
% \end{enumerate}
% \end{defn}
% \vspace{100pt}
% \begin{defn}
% Two modules (functors/representations) $\mathbf{F}$ and $\mathbf{G}$ are said to be $\vec{\varepsilon}$-interleaved if there exist a pair of natural transformations 
% $\varphi\colon \mathbf{F}\Rightarrow \mathbf{G}\Omega_{\vec{\varepsilon}}$ and 
% $\psi\colon \mathbf{G}\Rightarrow \mathbf{F}\Omega_{\vec{\varepsilon}}$ 
% such that the diagrams below commute.
% \vspace{70pt}
% We have
% \begin{itemize}
%     \item $\vec{\varepsilon}=(\varepsilon_1,\varepsilon_2)$;
%     \item $\Omega_{\vec{\varepsilon}}=\mathcal{T}_{\varepsilon_1}\circ \mathcal{U}_{\varepsilon_2}$.
% \end{itemize}
% The interleaving distance with respect to $\Omega_{\vec{\varepsilon}}$ is 
% \[
% d_{\Omega}(\mathbf{F},\mathbf{G})
% =\inf\set{\norm{\vec{\varepsilon}}_{\infty}|
% \text{
% $\mathbf{F}$ and $\mathbf{G}$ are $\vec{\varepsilon}$-interleaved
% }
% }.
% \]
% \end{defn}

% \vspace{20pt}

% \subsubsection{Barcodes and bottleneck distance}

% Let $\mathbf{M}$ be a commutative ladder module.
% \[
% \mathcal{B}(\mathbf{M})\coloneqq
% \set{\big(I,c_M^\xi(V_I)\big)}_{I\in\mathbb{I}}
% \]
% is a multiset.

% Define the bottleneck distance:
% \[
% d_B(\mathcal{\mathbf{F}},\mathcal{\mathbf{G}})
% =\inf\set{
% \norm{\vec{\varepsilon}}_{\infty}
% |
% \exists \text{ an $\vec{\varepsilon}$-matching between 
% $\mathcal{\mathbf{F}}$ and $\mathcal{\mathbf{G}}$.}
% }
% \]
% \newpage



==> legacy/legacy_stability_sec5/00541_stab.tex <==

\subsubsection{Induced Matchings of Connected Persistence Diagrams}

A connected persistence diagram contains multiple components that are not immediately comparable, and the multiplicity of a line segment in it can be negative in general cases. 
Compared with ordinary persistence diagrams, this lack of non-negativity presents a significant challenge that is beyond our current ability to handle. 
To make the task more manageable, we will assume the interval-decomposability condition. 
We will disassemble elements in a connected persistence diagram 
into three subsets and define a pseudo-distance on connected persistence diagrams by finding a matching between those sets separately.

% These are all obstacles to defining a bottleneck distance on connected persistence diagrams directly.


% Recall that the graph of a map $f\colon X\to Y$ is the set $G(f)\coloneqq \set{(x,f(x))|x\in X}$. Three sets will be created from the graph of a connected persistence diagram $\cPD$ and compared with their counterpart from another connected persistence diagram in parallel.
% where did i use that??

To ensure consistency with existing literature in stability theory, 
we will make slight adjustments to some of the notations previously introduced, 
aligning them with those used in \cite{bauer2013induced}. 
This will facilitate comparisons with related work and enable the extension of our results to a wider context.

All representations in this part are considered to be in the category $\rep(\cln)\subseteq \rep(\clinf)$
% interval-decomposable
unless explicitly stated otherwise.
\begin{defn}\label{defn:unpacking-map}
Let $M$ be an interval-decomposable representation and 
$\cPD(M)\colon \mathbb{I} \to \mathbb{Z}_{\geq 0}$ be the corresponding connected persistence diagram.
The \textit{unpacking map} $\mu$ maps $\cPD(M)$ to a tuple of three multisets that records horizontal persistence in the upper layer,
horizontal persistence in the lower layer, and width of the vertical persistence, respectively. 
Formally, we define $\mu\big(\cPD(M)\big)$ as follows:
\[
\mu\big(\cPD(M)\big) \coloneqq 
\big(
\prs{2}{\ca{B}},
\prs{1}{\ca{B}},
\prs{\layerV}{\ca{B}}
\big)
% \big(\prs{2}{\ca{B}}_M \prsss{2}{\ca{B}}{}{M} \prescript{2}{1}{\ca{B}}_M^N\prescript{2}{1}{\ca{B}}_M \ca{U},\ca{L},\ca{V}\big),
\]
where the underlying set and multiplicity function of each multiset is:
% superscripts: use 2,1 2/1 or u,l,v
\begin{itemize}
    %upper horizontal
    \item
    % Upper layer
    $\prs{2}{\ca{B}}=\big(\prs{2}{B},\prs{2}{\absv}\big)$ 
    with 
    $\prs{2}{B} = \set{\prs{2}{\iprod{b}{d}} | [b,d]_2\in \Iu}$ 
    and 
    $\prs{2}{\absv}\colon \prs{2}{\iprod{b}{d}}\mapsto \cPD(M)\big([b,d]_2\big)$.
    %lower horizontal
    \item $\prs{1}{\ca{B}}=\big(\prs{1}{B},\prs{1}{\absv}\big)$ 
    with 
    $\prs{1}{B}=\set{\prs{1}{\iprod{b}{d}} | [b,d]_1\in \Id}$ 
    and 
    $\prs{1}{\absv}\colon \prs{1}{\iprod{b}{d}}\mapsto \cPD(M)\big([b,d]_1\big)$.
    %vertical
    \item $\prs{\layerV}{\ca{B}}=\big(\prs{\layerV}{B},\prs{\layerV}{\absv}\big)$ 
    with 
    $\prs{\layerV}{B}=\set{\prs{\layerV}{\iprod{b_1}{d_2}} | [\cdotw,d_2]_2\sqcup [b_1,\cdotw]_1\in \Iud}$ 
    and 
    \[
    \prs{\layerV}{\absv}\colon \prs{\layerV}{\iprod{b_1}{d_2}}\mapsto \souwa{[b_2,d_2]_2\sqcup[b_1,d_1]_1\in \Iud}\cPD(M)\big([b_2,d_2]_2\sqcup[b_1,d_1]_1\big).
    \]
\end{itemize}
%
% \begin{itemize}
%     \item
%     $\ca{U}=\big(U,\absv^2\big)$ with $U=\set{\iprod{b}{d}^2 | [b,d]_2\in \Iu}$ 
%     and $\absv^2\colon \iprod{b}{d}^2\mapsto \cPD(M)\big([b,d]_2\big)$;
%     \item $\ca{L}=\big(L,\absv^1\big)$ with $L=\set{\iprod{b}{d}^1 | [b,d]_1\in \Id}$ 
%     and $\absv^1\colon \iprod{b}{d}^1\mapsto \cPD(M)\big([b,d]_1\big)$
%     \item $\ca{V}=\big(L,\absv^{\nicefrac{2}{1}}\big)$ with $V=\set{\iprod{b_1}{d_2}^{\nicefrac{2}{1}} | [\cdotw,d_2]_2\sqcup [b_1,\cdotw]_1\in \Iud}$ 
%     and 
%     \[
%     \absv^{\nicefrac{2}{1}}\colon \iprod{b_1}{d_2}^{\nicefrac{2}{1}}\mapsto \souwa{[b_2,d_2]_2\sqcup[b_1,d_1]_1\in \Iud}\cPD(M)\big([b_2,d_2]_2\sqcup[b_1,d_1]_1\big)
%     \]
%         % \item $U=\set{\big(I,\cPD(M)\big(I\big)\big)| I\in \Iu}=\set{\abte{b_2}{d_2}{m} | [b_2,d_2]_2\in \Iu, m=\cPD(M)\big([b_2,d_2]_2\big)}$;
%         % \item $L=\set{\big(I,\cPD(M)\big(I\big)\big)| I\in \Id}=\set{\abte{b_1}{d_1}{m} | [b_1,d_1]_1\in \Id, m=\cPD(M)\big([b_1,d_1]_1\big)}$;
%         % \item $V=\set{\abte{b_1}{d_2}{m} | b_1\leq d_2, m=\souwa{[b_2,d_2]_2\sqcup[b_1,d_1]_1\in \Iud}\cPD(M)\big([b_2,d_2]_2\sqcup[b_1,d_1]_1\big)}$.
% \end{itemize}
%
Notice that for intervals supported on both layers, only the overlapped parts are recorded and added together in the multiset $\prs{\layerV}{\ca{B}}$.
% \begin{enumerate}
%     \item Construct the following three multisets:
    
%     \item Initially, add all elements in $D_q^{\xi}(Y)$ to $U$ and all elements in $D_q^{\xi}(X)$ to $L$. Elements in them are guaranteed to have positive multiplicities.
%     \item For each $\big([b_1,d_1]_1\sqcup[b_2,d_2]_2,m\big)\in D_q^{\xi}(\substack{Y\\X})\Big)$, 
%     %add $\big([b_2,d_2]_2,m\big)$ to $U$,
%     %$\big([b_1,d_1]_1,m\big)$ to $L$,
%     %and $\big([b_1,d_2]_2\sqcup[b_1,d_2]_1,m\big)$ to $V$. 
%     add $\big([b_1,d_2]_1\sqcup[b_1,d_2]_2,m\big)$ to $V$. 
%     \item %Separate elements in the three multisets according to the positivity of their multiplicity. Write the result as
%     Separate elements in $V$ according to the positivity of their multiplicities. Write the set as a disjoint union:
%     \begin{itemize}
%         %\item $U=U^+\sqcup U^-$;
%         %\item $L=L^+\sqcup L^-$;
%         \item $V=V^+\sqcup V^-$.
%     \end{itemize}
%     \item Notice that an element $[b_1,d_2]_1\sqcup[b_1,d_2]_2$ in $V$ is guaranteed to have a rectangle shape, so it suffices to remove the redundant symbols and keep it as $\big([b_1,d_2],m)$, with the subscript ignored. We also ignore the subscripts of elements in $U$ and $L$ for simplicity.
%     \item Finally, $\mu(\cPD)$ is a tuple $\big(U,L,V^+,V^-\big)$, 
%     and an element in any of the sets can be written as $([b,d],m)$.
%     For simplicity, we further remove all redundant brackets and 
%     denote elements in form of $\abte{b}{d}{m}$.
%     % and an element in any of the set can be written as $([b,d],m)$.
%     % $\big(U^\pm,L^\pm,V^\pm\big)\coloneqq $
%     % $[b,d]_{\square}$
% \end{enumerate}
% It is easy to see that with the six multisets given above,
% a \textit{packing function} $\nu$ can be defined to retrieve original elements $\cPD$ by reconstructing  elements in $V$ first.
% No, it is not
% pack/unpacksadsdasds
% disassembly map
% assembly map
% uncouple/unpack
% cPD to two horizontal/vertical parts,
% further separated by positivity.
\end{defn}

\begin{rmk}
The left superscripts on the angled brackets are used to distinguish intervals from different layers, 
while the right subscripts are reserved for differentiating representations and the right superscripts for indicating operations. 
To avoid unnecessary repetition, we will ignore the left superscript in the multiplicity function of each multiset if it is clear from the context.
\end{rmk}

\begin{rmk}
Proposition \ref{prop:cPD-upper-lower-PD-equivalence} implies that 
elements in $\prs{2}{\ca{B}}$ and $\prs{1}{\ca{B}}$ correspond directly to birth-death pairs. 
That is, there is a one-to-one correspondence between $\prs{\square}{\iprod{b}{d}}$ and $[b,d]_{\square}$ 
for $\square\in{2,1}$. 
However, this statement does not hold for $\square=\nicefrac{2}{1}$. 
For example, if the intervals $[1,7]_2\sqcup [5,10]_1$ and $[4,7]_2\sqcup [5,8]_1$ 
both have multiplicity one under the map of $\cPD(M)$, 
then they each contribute one to the multiplicity of $\prs{\layerV}{\iprod{5}{7}}$ 
in $\prs{\layerV}{\ca{B}}$.
\end{rmk}


The operations utilized in proving the algebraic stability theorem of ordinary persistence diagrams have proven to be quite convenient \cite{bauer2013induced}. We now define their counterparts in $\mu\big(\cPD(M)\big)$ by vectorizing them.
\begin{defn}
Let $\cPD(M)$ be a connected persistence diagram where $M$ is an interval-decomposable representation,
$b$ and $d$ be two integers, $\delta$ be a non-negative integer.
We define the following operations on multisets 
$\big(\prs{2}{\ca{B}},\prs{1}{\ca{B}},\prs{\layerV}{\ca{B}}\big)=\mu\big(\cPD(M)\big)$. 
For each of these operations, we specify how the underlying set is modified, 
and the associated multiplicity function is meant to remain unchanged.

\begin{enumerate}
    \item Discarding intervals shorter than $\epsilon\in \mathbb{Z}_{\geq 0}$ for $\square \in \set{2,1,\nicefrac{2}{1}}$:
    \[
    \prs{\square}{\Lambda}^\epsilon\coloneqq (\prs{\square}{\Lambda})^\epsilon\coloneqq \set{\prs{\square}{\iprod{b}{d}}\in\prs{\square}{\Lambda}| d-b\geq \epsilon},
    \]
    where we set $\prs{2}{\Lambda}\coloneqq\prs{2}{B}$, 
    $\prs{1}{\Lambda}\coloneqq\prs{1}{B}$, 
    and $\prs{\layerV}{\Lambda}\coloneqq\prs{\layerV}{B}$.
    % Picking out intervals terminating at $d$
    \item Extracting intervals ending at $d$ for $\square \in \set{2,1,\nicefrac{2}{1}}$:
    \[
    \prs{\square}{\iprod{\cdotw}{d}}\coloneqq \set{\prs{\square}{\iprod{s}{t}}\in\prs{\square}{\Lambda})|t=d}.
    \]
    \item Extracting intervals starting from $b$ for $\square \in \set{2,1,\layerV}$:
    \[
    \prs{\square}{\iprod{b}{\cdotw}}\coloneqq \set{\prs{\square}{\iprod{s}{t}}\in\prs{\square}{\Lambda}|s=b}.
    \]
    \item If $I=[b,d]$ is an interval in $\Iu$ or $\Id$, selecting intervals ending at $d$ that contain $I$, or intervals starting from $b$ that contain $I$, for $\square \in \set{2,1}$:
    \[
    \begin{aligned}
    \prs{\square}{\iprod{\cdotw}{I}}&\coloneqq \set{J\supseteq I| J\in \prs{\square}{\iprod{\cdotw}{d}}}\\
    \prs{\square}{\iprod{I}{\cdotw}}&\coloneqq \set{J\supseteq I| J\in \prs{\square}{\iprod{b}{\cdotw}^\square}}
    \end{aligned}
    \]
    \item If $I=[b_2,d_2]_2\sqcup[b_1,d_1]_1\in \Iud$, selecting intervals ending at $d_2$ in the upper layer that contain $I$,
    or intervals starting from $b_1$ in the lower layer that contain $I$:
    \[
    \begin{aligned}
    \prs{\layerV}{\iprod{\cdotw}{I}}&\coloneqq \set{J\supseteq I | J\in \prs{\layerV}{\iprod{\cdotw}{d_2}}}\\
    \prs{\layerV}{\iprod{I}{\cdotw}}&\coloneqq \set{J\supseteq I | J\in \prs{\layerV}{\iprod{b_1}{\cdotw}}}\\
    \end{aligned}
    \]
    \item A shorthand notation for operation 1 defined at the tuple level for $\epsilon\in\mathbb{Z}_{\geq 0}$:
    \[
        \mu\big(\cPD(M)\big)^{\epsilon} \coloneqq 
        \big(\prs{2}{\ca{B}}^{\epsilon},\prs{1}{\ca{B}}^{\epsilon},\prs{\layerV}{\ca{B}}^{\epsilon})\\
    \]
    % \item Operation 1 defined at the tuple level for $\vdel=(\delta_1,\delta_2)$:
    % \[
    %     \mu\big(\cPD(M)\big)^{\vdel} \coloneqq 
    %     \big(\prs{2}{\ca{B}}^{\delta_2+\delta_1},\prs{1}{\ca{B}}^{\delta_1},\prs{\layerV}{\ca{B}}^{\delta_2})\\
    % \]
    \item 
    Shorthand notations for operations 2-5 defined at the tuple level:
    \[
    \begin{aligned}
    \prs{{\mu(\cPD(M))}}{\rectangle}&\coloneqq \big(\prs{2}{\rectangle},\prs{1}{\rectangle},\prs{\layerV}{\rectangle})
    &\mbox{for } \rectangle \in 
    \set{\iprod{\cdotw}{d},\iprod{b}{\cdotw},\iprod{\cdotw}{I},\iprod{I}{\cdotw}}.
    \end{aligned}
    \]    
\end{enumerate}

We can use these operations to establish a lexicographical order based on the reverse inclusion relations of 
the birth-death pairs and the values of the multiplicities. 
This allows us to arrange the features according to their significance.

For $ \square \in \set{2,1,\nicefrac{2}{1}}$, equip $\prs{\square}{\iprod{\cdotw}{d}}$ with the following partial order:
\begin{itemize}
    \item $\prs{\square}{\iprod{s}{d}}<\prs{\square}{\iprod{s'}{d}}$ if and only if $s<s'$.
    % , or $s=s'$ and $\abs{\iprod{s}{d}^{\square}}>\abs{\iprod{s'}{d}^{\square}}$.
\end{itemize}
Similarly, the partial order defined on $\prs{\square}{\iprod{b}{\cdotw}}$ is:
\begin{itemize}
 \item $\prs{\square}{\iprod{b}{t}}<\prs{\square}{\iprod{b}{t'}}$ if and only if $t>t'$.
 % , or $t=t'$ and $\abs{\iprod{b}{t}^{\square}}>\abs{\iprod{b}{t'}^{\square}}$.
\end{itemize}
\end{defn}



% A distance on the set of connected persistence diagrams will be defined via the use of the unpacking function.
We can extend the definition of a matching between two sets to matchings between two tuples of sets.
Recall that a matching $\sigma$ between two sets $A$ and $B$ (written as $\sigma\colon A\centernot\rightarrow B$) is a bijection between $A'\subseteq A$ and $B'\subseteq B$,
where $A'$ is denoted as $\Coim\sigma$ and $B'$ is denoted as $\Im\sigma$.
Let $\vv{A}\coloneqq (A_1, \dots, A_n)$ and $\vv{B}\coloneqq(B_1, \dots, B_n)$ be two tuples of sets, 
we define a \textit{tuple of matchings} $\vv{\sigma} = (\sigma_1, \dots, \sigma_n)$ between $\vv{A}$ and $\vv{B}$ 
to be a collection of matchings such that each $\sigma_i$ is a matching between $A_i$ and $B_i$ for each $i \in \set{1, \dots, n}$. 
We use $\Coim\vv{\sigma}$ and $\Im\vv{\sigma}$ to denote the tuples of sets where the $\Coim$ or $\Im$ operations are applied element-wisely.


% Next, the definition of matching between two sets is vectorized to matchings between two tuples of sets.
% Recall that a matching $\sigma$ between two sets $A$ and $B$ (written as $\sigma\colon A\centernot\rightarrow B$) is a bijection between $A'\subseteq A$ and $B'\subseteq B$,
% where $A'$ is denoted as $\Coim\sigma$ and $B'$ is denoted as $\Im\sigma$.
% We say $\vv{\sigma}=(\sigma_1,\cdots,\sigma_n)$ is a \textit{tuple of matchings} between tuples of sets $(A_1,\cdots,A_n)$ and 
% $(B_1,\cdots,B_n)$ if each $\sigma_i$ is a matching
% between $A_i$ and $B_i$.
% $\Coim\vv{\sigma}$ and $\Im\vv{\sigma}$ denote tuples of sets where the operations are applied element-wisely.
% We define a matching $\vv{\sigma}$ between two tuples of multisets 
% $(S_i)_{i\in I}$ and $(T_i)_{i\in I}$
% to be a tuple of matchings $(\sigma_i)_{i\in I}$,
% where each $\sigma_i$ is a matching between $S_i$ and $T_i$.
\begin{defn}[$\delta$-matching] % definition above remark 3.3 in the reference % the coefficient 2 comes from there
Given two interval-decomposable representations $M$ and $N$, 
let $D_M\coloneqq\cPD(M)$ and $D_N\coloneqq\cPD(N)$ denote their connected persistence diagrams, respectively.
A \textit{$\delta$-matching} between $D_M$ and $D_N$ 
is a tuple of matchings 
$\vv{\sigma}=
\big(
\sigma_{2},
\sigma_{1},
\sigma_{\layerV}
\big)$ 
between multisets in $\mu(D_M)=(\prs{2}{B}_M,\prs{1}{B}_M,\prs{\layerV}{B}_M)$ 
and $\mu(D_N)=(\prs{2}{B}_N,\prs{1}{B}_N,\prs{\layerV}{B}_N)$
such that 
\[
\mu(D_M)^{2\delta}\subseteq \Coim\vv{\sigma}
\qquad
\mbox{and}
\qquad
\mu(D_N)^{2\delta}\subseteq \Im\vv{\sigma},
\]
where the inclusions are meant to be evaluated element-wisely.
In addition, we require that for all $\sigma_\square(\prs{\square}{\iprod{b}{d}})=\prs{\square}{\iprod{b'}{d'}}$, 
the following two inequalities hold:
\[
b'-\delta\leq b\leq d\leq d'+\delta,
\qquad
b-\delta\leq b'\leq d'\leq d+\delta.
\]
Two connected persistence diagrams are said to be 
\textit{$\delta$-matched} if there exists a $\delta$-matching 
between them.
\end{defn}
\begin{figure}[H]
    \centering
    \begin{tikzpicture}
% Draw the real line
\draw (-2.5,0) -- (2.5,0);

% \filldraw [black] (-1.5,0) circle (2pt);
% \filldraw [black] (1.5,0) circle (2pt);
% Draw the labels below the line
\node[below] at (-1.5,0) {$b$};
\node[below] at (1.5,0) {$d$};
% % Draw the shaded region around b
\fill[gray!40,opacity=0.618] (-1.6-0.3,0.1) rectangle (-1.6+0.3,-0.1);
% Draw the label above the shaded region
\node[above] at (-1.5,0.2) {$\langle b'-\delta,b'+\delta\rangle$};
% Draw the shaded region around d
\fill[gray!40,opacity=0.618] (1.6-0.3,0.1) rectangle (1.6+0.3,-0.1);
% Draw the label above the shaded region
\node[above] at (1.5,0.2) {$\langle d'-\delta,d'+\delta\rangle$};
% Draw the vertical lines to illustrate the location of b and d
\draw[solid, line width=1pt] (-1.5,0.1) -- (-1.5,-0);
\draw[solid, line width=1pt] (1.5,0.1) -- (1.5,-0);
\end{tikzpicture}
    \caption{Illustration of relative positions between $\langle b,d\rangle$ and $\langle b',d'\rangle$. Each gray area represents its corresponding interval written on the top.}
    \label{fig:bdbpdp-relation}
\end{figure}


\begin{defn}[Bottleneck Distance]
Let 
Let $D_M\coloneqq\cPD(M)$ and $D_N\coloneqq\cPD(N)$ be two connected persistence diagrams
of two interval-decomposable representations $M$ and $N$.
The \textit{bottleneck distance} between $D_M$ and $D_N$ 
is
\[
d_B(D_M,D_N)\coloneqq 
\inf\set{\delta\in \mathbb{Z}_{\geq 0}|
\text{
$D_M$ and $D_N$ are $\delta$-matched}
}.
\]
\end{defn}

\begin{prop}
The bottleneck distance defined above is a pseudometric on the set of connected persistence diagrams.
\begin{proof}
    Reflexivity and symmetry are easily verifiable using the definition.
    One property that may not be immediately obvious is triangle inequality. To prove this, consider two matchings: $\vv{\sigma}_1$, a $\delta_1$-matching between $D$ and $D'$; and $\vv{\sigma}_2$, a $\delta_2$-matching between $D'$ and $D''$. It can be shown that the element-wise composition of these matchings is a $(\delta_1 + \delta_2)$-matching between $D$ and $D''$, from which the desired result follows.
\end{proof}
\end{prop}


%canonical matching
Recall that if $S=\set{s_j|j=1,\cdots,|S|}$ and $T=\set{t_j|j=1,\cdots,|T|}$ are two finite totally ordered sets with partial orders both inferred from the subscripts (as a poset in $\mathbb{N}$), 
then a \textit{canonical matching} $\sigma\colon S\centernot\rightarrow T$ is defined by $\sigma(s_j)=t_j$ for $j=1,\cdots,\min\set{s,t}$, from which we have $\Coim\sigma=S$ or $\Im\sigma =T$. This concept can be extended to the case of tuples of sets. Let
\[
\vv{S}=(S^1,\cdots,S^m)\qquad
\vv{T}=(T^1,\cdots,T^m)
\]
be two tuples of finite totally ordered sets where $S^i=\set{s^i_j|j=1,\cdots,|S^i|}$ and $T^i=\set{t^i_j|j=1,\cdots,|T^i|}$.
A \textit{canonical matching} $\vv{\sigma}\colon \vv{S}\centernot\rightarrow\vv{T}$ is a tuple of canonical matchings $(\sigma^1,\ldots,\sigma^m)$ where each $\sigma^i$ is a canonical matching between $S^i$ and $T^i$.
With this vectorized version of canonical matching, we can now define the induced matching between connected persistence diagrams.

\begin{defn}[Induced Matching]\label{defn:induced-matching}
Let $f\colon M\to N$ be a morphism between two interval-decomposable representations,
and let $D_M\coloneqq\cPD(M)$ and $D_N\coloneqq\cPD(N)$ be the corresponding connected persistence diagrams.
The induced matching 
\[
\chi_f
% \mu(f)
\colon \mu(D_M) \centernot\rightarrow \mu(D_N)
\]
is defined following the descriptions below.
\begin{enumerate}
    \item If $f$ is injective, $\chi_f$ is the tuple of canonical matchings from 
    $\prs{^{\mu(D_M)}}{\iprod{\cdotw}{d}}_M$
    to
    $\prs{^{\mu(D_N)}}{\iprod{\cdotw}{d}}_N$.
    \item If $f$ is surjective, $\chi_f$ is the tuple of canonical matchings from 
    $\prs{\mu(D_M)}{\iprod{b}{\cdotw}}_M$
    to
    $\prs{\mu(D_N)}{\iprod{b}{\cdotw}}_N$.
    \item In the general case, decompose $f$ as the composition of the following two maps:
    \[
    \begin{tikzcd}[column sep=normal]
    M \arrow[r,two heads,"q_f"] &\Im f \arrow[r,hook,"j_f"] & N
    \end{tikzcd}
    \]
    where $q_f$ is surjective and $j_f$ is injective.
    Then we define $\chi_f$ to be the composition of the induced matchings $\chi_{j_f}\circ\chi_{q_f}$.
    
\end{enumerate}
\end{defn}

It is desirable for $\Coim \chi_f$ to be equal to $\prs{^{\mu(D_M)}}{\iprod{\cdotw}{d}}_M$ when $f$ is injective, 
and for $\Im \chi_f$ to be equal to $\prs{\mu(D_N)}{\iprod{b}{\cdotw}}_N$ when $f$ is surjective. 
Theorem \ref{thm:structure_thm_interval-decomposable_cPD} establishes this result as a generalization of \cite[Theorem 4.2]{bauer2013induced}
in the context of commutative ladders. The following lemma is used in the proof of that theorem.
% Below we have the structure theorem for connected persistence diagrams

\begin{lemma}\label{lemma:stability-thm-key-lemma-inequality}%lemma4.3 in \cite{bauer2013induced}
Let $f\colon M\to N$ be a homomorphism between interval-decomposable representations. For any interval $I\in \Iud$, we have:
\begin{enumerate}
    \item If $f$ is a monomorphism, then $\abs{\prs{\layerV}{\iprod{\cdotw}{I}_M}} \leq \prs{\layerV}{\abs{\iprod{\cdotw}{I}}_N}$.
    \item If $f$ is an epimorphism, then $\abs{\prs{\layerV}{\iprod{\cdotw}{I}_M}} \geq \prs{\layerV}{\abs{\iprod{\cdotw}{I}}_N}$.
\end{enumerate}

\begin{proof}
Denote the interval $I$ as $[b_2,d_2]_2\sqcup [b_1,d_1]_1$.
According to the definition, the following equations hold: % notice that b_2, d_2 are fixed.
\[
\begin{aligned}
\abs{\prs{\layerV}{\iprod{\cdotw}{I}}_M} = \souwa{[s_2,d_2]_2\sqcup[s_1,t_1]_1\supseteq I}\cPD(M)\big([s_2,d_2]_2\sqcup [s_1,t_1]_1\big),\\
\abs{\prs{\layerV}{\iprod{\cdotw}{I}}_N} = \souwa{[s_2,d_2]_2\sqcup[s_1,t_1]_1\supseteq I}\cPD(N)\big([s_2,d_2]_2\sqcup [s_1,t_1]_1\big),\\
\abs{\prs{\layerV}{\iprod{I}{\cdotw}}_M} = \souwa{[s_2,t_2]_2\sqcup[b_1,t_1]_1\supseteq I}\cPD(M)\big([s_2,t_2]_2\sqcup[b_1,t_1]_1\big),\\
\abs{\prs{\layerV}{\iprod{I}{\cdotw}}_N} = \souwa{[s_2,t_2]_2\sqcup[b_1,t_1]_1\supseteq I}\cPD(N)\big([s_2,t_2]_2\sqcup[b_1,t_1]_1\big).
\end{aligned}
\]
% Recall that if $I$ is an interval, then $V_I$ denotes its associated interval representation (see remark \ref{rmk:interval-and-interval-representation}).
\begin{enumerate}
    \item 
    As $f$ is injective, % f applies on the interval
    it suffices to show that for each interval representation that contributes to the sum of $\abs{\prs{\layerV}{\iprod{\cdotw}{I}}_M}$, we can find an associated interval representation that contributes the sum $\abs{\prs{\layerV}{\iprod{\cdotw}{I}}_N}$. This amounts to proving the following statement: 
    % By the equations above, a
    \begin{itemize}
    \item For each $I'=\intvV{s_2}{d_2}{s_1}{t_1}\supseteq I$ such that $V_{I'}$ is a direct summand of $M$ 
    (so ${\cPD(M)\big(I'\big) >0}$), $f(V_{I'})$ is contained in some $V_{\tilde{I}}$ where $\tilde{I}\supseteq I$ is of form ${\intvV{\cdotw}{d_2}{\cdotw}{\cdotw}}$.
    \end{itemize}
    As $N$ is interval-decomposable, $f(V_{I'})$ has to be contained in an interval representation $V_{\tilde{I}}$. 
    Immediately we have $\tilde{I}\supseteq I$ since $f$ is injective.
    Denote $\tilde{I}$ as $\intvV{x_2}{y_2}{x_1}{y_1}$.
    First we notice that $(V_{I'})_{(d_2,2)}=\Bbbk$, thus $f\big((V_{I'})_{(d_2,2)}\big)\neq \mathbf{0}$ as $f$ is injective,
    this shows that $y_2\geq d_2$. For the other direction, we notice that the following diagram has to be commutative for each $y_2 > d_2$:
    \[
    \begin{tikzcd}
    (V_{I'})_{(d_2,2)}\arrow[r,"\varphi"]\arrow[d,"f"']&(V_{I'})_{(y_2,2)}\arrow[d,"f"]\\
    (V_{\tilde{I}})_{(d_2,2)}\arrow[r,"\varphi"]&(V_{\tilde{I}})_{(y_2,2)}.
    \end{tikzcd}
    \]
    Note that $f\circ \varphi=0$ since $(V_{I'})_{(y_2,2)}=\mathbf{0}$ if $y_2>d_2$, thus by commutativity $\varphi\circ f=0$. If $(V_{\tilde{I}})_{(y_2,2)}$ is non-zero, 
    then $f=0$ because $\varphi$ will be a transition map, which is injective. This is a contradiction, so
    $(V_{\tilde{I}})_{(y_2,2)}$ has to be $\mathbf{0}$.
    This finishes the proof that $y_2=d_2$ (in fact, we can also prove that $y_1=t_1$ in the same fashion).
    \item For this dual statement, it suffices to prove the following statement:
    \begin{itemize}
        \item For each $I'=\intvV{s_2}{t_2}{b_1}{t_1}\supseteq I$ such that $V_{I'}$ is a direct summand of $N$ 
    (so ${\cPD(N)\big(I'\big) >0}$), 
    there exists a $V_{\tilde{I}}$ being a direct summand of $M$ such that $f(V_{\tilde{I}})\supseteq V_{I'}$
    (since $f$ is subjective).
    Then $\tilde{I}$ is of form ${\intvV{\cdotw}{\cdotw}{b_1}{\cdotw}}$ and $\tilde{I}\supseteq I$.
    \end{itemize}
    Assume $\tilde{I}$ is of form $\intvV{x_2}{y_2}{x_1}{y_1}$. As $f$ is surjectively and $f(V_{\tilde{I}})\supseteq V_{I'}$, $x_1\leq b_1$.
    The other direction can be proved similarly as in the previous point by considering the following diagram for $x_1<b_1$:
    \[
    \begin{tikzcd}
    (V_{\tilde{I}})_{(x_1,1)}\arrow[r,"\varphi"]\arrow[d,"f"']&(V_{\tilde{I'}})_{(b_1,1)}\arrow[d,"f"]\\
    (V_{I'})_{(x_1,1)}\arrow[r,"\varphi"]&(V_{I'})_{(b_1,1)}.
    \end{tikzcd}
    \]
    We know that $\varphi\circ f = 0$ as $(V_{I'})_{(x_1,1)}=\mathbf{0}$, thus $f\circ \varphi=0$ by commutativity. This requires $(V_{\tilde{I}})_{(x_1,1)}$ to be $\mathbf{0}$, otherwise $f=0$ because $\varphi$ is surjective.
    %
    Given that $\varphi\circ f = 0$ as $(V_{I'}){(x_1,1)}=\mathbf{0}$, it follows by commutativity that $f\circ \varphi=0$. This means $(V_{\tilde{I}})_{(x_1,1)}$ must also be $\mathbf{0}$, otherwise $\varphi$ would be subjective, from which we can deduce $f=0$, a contradiction. Thus $x_1=b_1$.
\end{enumerate}
\end{proof}
\end{lemma}

\begin{thm}\label{thm:structure_thm_interval-decomposable_cPD}%[Structure of persistence submodules and quotients]
Let $M,N$ be two interval-decomposable representations and the corresponding connected persistence diagrams be $D_M\coloneqq \cPD(M)$ and $D_N\coloneqq \cPD(N)$.
\begin{enumerate}
    \item If there exists a monomorphism $M\hookrightarrow N$, then for each $d\in\set{1,\cdots,n}$ and $\square\in \set{2,1,\layerV}$,
    \[
    \abs{\prs{\square}{\iprod{\cdotw}{d}}_M} \leq \abs{\prs{\square}{\iprod{\cdotw}{d}}_N}
    \]
    and the canonical injection $\chi_f\colon \mu(D_M)\hookrightarrow \mu(D_N)$ maps each $\prs{\square}{\iprod{b}{d}}$ to 
    $\prs{\square}{\iprod{b'}{d}}$ with $b'\leq b$.
    \item Dually, if there exists an epimorphism $M\twoheadrightarrow N$, then for each $b\in\set{1,\cdots,n}$ an $\square \in \set{2,1,\layerV}$,
    \[
    \abs{\prs{\square}{\iprod{b}{\cdotw}}_M}\geq \abs{\prs{\square}{\iprod{b}{\cdotw}}_N}
    \]
    and the canonical surjection $\chi_f\colon \mu(D_M)\twoheadrightarrow \mu(D_N)$ 
    satisfies $\chi_f^{-1}(\prs{\square}{\iprod{b}{d}})=\prs{\square}{\iprod{b}{d'}}$ where $d \leq d'$.
    
\end{enumerate}
\begin{proof}
The results for $\square\in\set{2,1}$ follow from Proposition \ref{prop:cPD-upper-lower-PD-equivalence} 
and \cite[Theorem 4.2]{bauer2013induced}.
We prove the statements for the case $\square=\layerV$.
\begin{enumerate}
    \item To prove the inequality in the statement, it suffices to show that for any $i\leq \abs{\prs{\layerV}{\iprod{\cdotw}{d}}_M}$, it implies $i\leq \abs{\prs{\layerV}{\iprod{\cdotw}{d}}_N}$.
    Recall that elements in $\prs{\layerV}{\iprod{\cdotw}{d}}_M$ is of form $\prs{\layerV}{\iprod{b}{d}}$ for some $b\leq d$ and this multiset has a partial order.
    Denote the $i$-th element in $\prs{\layerV}{\iprod{\cdotw}{d}}_M$ as $I=\prs{\layerV}{\iprod{b}{d}}$ (counting the multiplicities).
    Then for $j$ within range $1\leq j\leq i$, $\prs{\layerV}{\iprod{\cdotw}{I}}_M$ contains the $j$-th 
    % interval 
    element of 
    $\prs{\layerV}{\iprod{\cdotw}{d}}_M$, because the $j$-th element of 
    $\prs{\layerV}{\iprod{\cdotw}{d}}_M$ is of form 
    $\prs{\layerV}{\iprod{x}{d}}$ with some $x\leq b$, 
    thus $\prs{\layerV}{\iprod{x}{d}}\supseteq I$. So the following inequalities hold:
    \[
    i\leq\abs{\prs{\layerV}{\iprod{\cdotw}{I}}_M}\leq 
    \abs{\prs{\layerV}{\iprod{\cdotw}{I}}_N}\leq 
    \abs{\prs{\layerV}{\iprod{\cdotw}{d}}_N},
    \]
    where the first inequality is by the choice of $I$, 
    the second one by lemma \ref{lemma:stability-thm-key-lemma-inequality}, 
    and the third one by the definition of $\prs{\layerV}{\iprod{\cdotw}{d}}_N$.
    For the canonical matching, we note that $I$ is mapped to $I'$ 
    where $I'$ is the $i$-th element of $\prs{\layerV}{\iprod{\cdotw}{d}}_N$.
    We want to prove that 
    $I'\in \prs{\layerV}{\iprod{\cdotw}{I}_N}$, which is obvious since
    $\prs{\layerV}{\abs{\iprod{\cdotw}{I}}}_M \leq \abs{\prs{\layerV}{\iprod{\cdotw}{I}}}_N$, 
    and $\chi_f$ matches from the longest element,
    so the $i$-the element of $\prs{\layerV}{\iprod{\cdotw}{d}}_N$ 
    is still in $\prs{\layerV}{\iprod{\cdotw}{I}}_N$.

    %epimorphism
    \item 
    This statement can be proved in a dual fashion. First we prove that for any ${\abs{\prs{\layerV}{\iprod{b}{\cdotw}}_N}\geq i}$,
    ${\abs{\prs{\layerV}{\iprod{b}{\cdotw}}_M}\geq i}$.
    Denote the $i$-th element of 
    $\prs{\layerV}{\iprod{b}{\cdotw}}_N$ as $I=\prs{\layerV}{\iprod{b}{d}}$.
    Then for $1\leq j\leq i$, $\prs{\layerV}{\iprod{I}{\cdotw}}_N$ 
    contains the $j$-th element of $\prs{\layerV}{\iprod{b}{\cdotw}}_N$
    (the $j$-th element is of form $\prs{\layerV}{\iprod{b}{y}}$, 
    and by the partial order we have $d\leq y$). Thus
    \[
    \abs{\prs{\layerV}{\iprod{b}{\cdotw}}_M}\geq
    \abs{\prs{\layerV}{\iprod{I}{\cdotw}}_M}\geq
    \abs{\prs{\layerV}{\iprod{I}{\cdotw}}_N},
    \]
    by parallel arguments as in the previous proof.
    For the canonical matching, $I$ is the image of the $i$-th element of $\prs{\layerV}{\iprod{b}{\cdotw}}_M$, denoted as $I'$.
    We want to show that $I'\in \prs{\layerV}{\iprod{I}{\cdotw}}_M$. The argument follows similarly as in the previous case
    since $\abs{\prs{\layerV}{\iprod{I}{\cdotw}}_M}\geq\abs{\prs{\layerV}{\iprod{I}{\cdotw}}_N}$.
\end{enumerate}
\end{proof}
\end{thm}


%prop 5.4, 5.5 not needed

We demonstrate some properties of induced matchings that will be used in the next part.

%prop 5.3
%\leq in the middle compared with < in the reference
\begin{prop}\label{prop:relations-between-births-and-deaths}
Let $f\colon M\to N$ be a morphism between interval-decomposable objects 
% in $\rep(\cln)\subseteq\rep(\clinf)$
and suppose $\chi_f(\prs{\square}{\iprod{b}{d}})=\prs{\square}{\iprod{b'}{d'}}$ for $\square\in \set{2,1,\layerV}$. Then
\[
b'\leq b\leq d'\leq d
\]
\begin{proof}
By Definition \ref{defn:induced-matching},
$\chi_f(\prs{\square}{\iprod{b}{d}})
=\chi_{j_f}\circ\chi_{q_f}(\prs{\square}{\iprod{b}{d}})
=\chi_{j_f}(\prs{\square}{\iprod{b}{d'}})
=\prs{\square}{\iprod{b'}{d'}}$
with $d'\leq d$ and $b'\leq b$, where the last two equations are by Theorem \ref{thm:structure_thm_interval-decomposable_cPD}.
\end{proof}
\end{prop}

\begin{prop}\label{prop:partial_functorial_induced_matching} %prop 5.7 in the reference
The operation $\chi$ is functorial on monomorphisms and epimorphisms in $\cat{rep}(\cln)$.
\begin{proof}
If $\id\colon M\to M$ is the identity map, then $\chi_{\id}$ is obviously the identity map $\mu\big(\cPD(M)\big)\to \mu\big(\cPD(M)\big)$.
Consider the composition of morphism $L\xrightarrow{g}M\xrightarrow{f}N$. 
If both $f$ and $g$ are injective, then ${\abs{\prs{\square}{\iprod{\cdotw}{d}}_L}}\leq {\abs{\prs{\square}{\iprod{\cdotw}{d}}_M}}\leq {\abs{\prs{\square}{\iprod{\cdotw}{d}}_N}}$ by Theorem \ref{thm:structure_thm_interval-decomposable_cPD}, thus $\chi_{f\circ g}=\chi_f\circ \chi_g$ by the definition of canonical matching. A dual argument proves the statement for epimorphisms.
\end{proof}

\end{prop}

% do we need prop 5.5?
%dual property:
% if $f\colon M\to N$ is injective, then $f^*$ is surjective


==> legacy/legacy_stability_sec5/00542_stab.tex <==


\subsubsection{Algebraic Stability via Induced Matchings}

Following the preparing works, 
in this part we prove the induced matching theorem 
and use it to prove an algebraic stability theorem.
All representations are considered to be in the category ${\rep(\cln)\subseteq \rep(\clinf)}$ as well.

% introduction about what's being done in this part
% Four ss-vertices lemma
\colorbox{red}{where did i use ss? }
\begin{lemma}\label{lemma:cPD-four-ss-vertices}
Let $M$ be an interval-decomposable representation, 
$\vec{\delta}=(\delta_1,\delta_2)\in \mathbb{Z}^2_{\geq 0}$, 
$\xi^{\operatorname{ss}}$ be the source-sink type assignment, 
$D_M\coloneqq \cPD^{\xi^{\operatorname{ss}}}(M)$ and $D_{M(\vdel)}\coloneqq \cPD^{\xi^{\operatorname{ss}}}\big(M(\vdel)\big)$
be the corresponding connected persistence diagrams.
Denote the multisets generated by the unpacking maps as
\[
\mu(D_{M(\vdel)})=
\big(
\prs{2}{\ca{B}}_{M(\vdel)},
\prs{1}{\ca{B}}_{M(\vdel)},
\prs{\layerV}{\ca{B}}_{M(\vdel)}
\big)
% \big(U_{\vdel},L_{\vdel},V_{\vdel}\big)
\qquad \mbox{and}
\qquad
\mu(D)=\big(
\prs{2}{\ca{B}}_M,
\prs{1}{\ca{B}}_M,
\prs{\layerV}{\ca{B}}_M
\big).
\]
Then there exists a $\norm{\vdel}_{1}$-matching 
\[
\vv{\rho}_M
\coloneqq 
(\rho_2,\rho_1,\rho_{\layerV})
\colon 
\mu(D_{M(\vdel)})
\centernot\rightarrow
\mu(D_M),
\]
where each component in the tuple is defined as:
\[
    \begin{aligned}
    %U
        \rho_2 \colon \prs{2}{\ca{B}}_{M(\vdel)} &\to \prs{2}{\ca{B}}_M\\
        \prs{2}{\iprod{b}{d}}&\mapsto \prs{2}{\iprod{b+\delta_1+\delta_2}{d+\delta_1+\delta_2}},\\
    %L
        \rho_1 \colon \prs{1}{\ca{B}}_{M(\vdel)} &\to \prs{1}{\ca{B}}_M\\
        \prs{1}{\iprod{b}{d}}&\mapsto \prs{1}{\iprod{b+\delta_1}{d+\delta_1}},\\
    %V
        \rho_{\layerV} \colon \prs{\layerV}{\ca{B}}_{M(\vdel)} &\to \prs{\layerV}{\ca{B}}_M\\
        \prs{\layerV}{\iprod{b}{d}}&\mapsto \prs{\layerV}{\iprod{b+\delta_1}{d+\delta_1+\delta_2}}.
    \end{aligned}
\]
\begin{proof}
We prove the expressions for the three matchings, then show that $\vv{\rho}_M$ is indeed a $\norm{\vdel}_1$-matching.

\noindent\textbf{Proof for $\rho_2$ and $\rho_1$:}

% \noindent 
Recall that $M(\vdel)=\ca{T}_{\vdel}(M)=\ca{H}_2(\delta)\circ\ca{H}_1(\delta_1)(M)$.
It is easy to see that the sole effect of functor $\ca{T}_{\vdel}$ on the two (ordinary) persistence diagrams $\PD\big(\overline{M}\big)$ and 
$\PD\big(\underline{M}\big)$ is an index translation. Specifically, we have
\[
\begin{aligned}
\PD\big(\overline{M(\vdel)}\big)\big([b,d]\big)&=\PD\big(\overline{M}\big)\big([b+\delta_1+\delta_2,d+\delta_1+\delta_2]\big),\\
\PD\big(\underline{M(\vdel)}\big)\big([b,d]\big)&=\PD\big(\underline{M}\big)\big([b+\delta_1,d+\delta_1]\big).
\end{aligned}
\]
Then it follows from proposition \ref{prop:cPD-upper-lower-PD-equivalence} that $D_{M(\vdel)}\big|_{\Iu}$ and $D_{M(\vdel)}\big|_{\Id}$ can also be derived from $D_M\big|_{\Iu}$ and $D_M\big|_{\Id}$ via a same index translation. The expressions for $\rho_2$ and $\rho_1$ follow naturally from the canonical matchings.

\noindent\textbf{Proof for $\rho_{\layerV}$:}

% \noindent
We group the interval summands of $M$ as $M\cong \prs{2}{M}\oplus\prs{1}{M}\oplus\prs{\layerV}{M}$, 
\textcolor{red}{used interval-decomposability here}
where $\prs{\square}{M}=\Directsum{I\in\mathbb{I}_{\square}}V_I^{d_M(V_I)}$. 
Consider an interval $I=[c_2,e_2]_2\sqcup[c_1,e_1]_1$ and $V_I$ being a direct summand of $\prs{\layerV}{M}$.
After the translation, we have
\[
\begin{aligned}
V_I(\vdel)_{(x,y)}
&=
\begin{cases}
    (V_I)_{(x+\delta_1+\delta_2,2)} & y=2\\
    (V_I)_{(x+\delta_1,1)} & y=1\\
\end{cases}
=
\begin{cases}
    \mathbb{k} & c_2\leq x+\delta_1+\delta_2\leq e_2,\ y=2\\
    \mathbb{k} & c_1\leq x+\delta_1\leq e_1,\ y=1\\
    \mathbf{0} & \mbox{otherwise}\\
\end{cases}\\
&
=
\begin{cases}
    \mathbb{k} & c_2-\delta_1-\delta_2\leq x\leq e_2-\delta_1-\delta_2,\ y=2\\
    \mathbb{k} & c_1-\delta_1\leq x \leq e_1-\delta_1,\ y=1\\
    \mathbf{0} & \mbox{otherwise}\\
\end{cases},
\end{aligned}
\]
where the transition morphism between any adjacent non-zero vector spaces is $\id_{\mathbb{k}}$,
so there exists a non-zero vertical map if and only if $c_1-\delta_1\leq e_2-\delta_1-\delta_2$, 
\textit{i.e.} $e_2-c_1\geq \delta_2$. This allows us to express $V_I(\vdel)$ in a more explicit form:
\[
V_I(\vdel)\cong
\begin{cases}
V_{[c_2-\delta_1-\delta_2,e_2-\delta_1-\delta_2]_2\sqcup[c_1-\delta_1,e_1-\delta_1]_1} & e_2-c_1\geq \delta_2\\
V_{[c_2-\delta_1-\delta_2,e_2-\delta_1-\delta_2]_2}\oplus V_{[c_1-\delta_1,e_1-\delta_1]_1} & e_2-c_1< \delta_2\\
\end{cases}.
\]
This condition prompts us to set up an overlapped width function for intervals in $\Iud$:
% has no restriction on the location of the interval. can translate
\[
\begin{aligned}
\omega:\Iud &\to \mathbb{Z}\\
I=[c_2,e_2]_2\sqcup[c_1,e_1]_1 &\mapsto e_2-c_1.
\end{aligned}
\]
Now we turn to obtain the required decomposition of $M(\vdel)$.
Notice that it is still interval-decomposable, and the decomposition of $\prs{\layerV}{\big(M(\vdel)\big)}$
as intervals can be obtained by applying $\ca{T}_{\vdel}$ on the interval decomposition of $\prs{\layerV}{M}$:
\[
\begin{aligned}
\ca{T}_{\vdel}\big(\prs{\layerV}{M}\big)
&=
\ca{T}_{\vdel}\big(
\Directsum{I\in\mathbb{I}_{\layerV}}V_I^{d_M(V_I)}
\big)\\
&=\Directsum{I\in\mathbb{I}_{\layerV}}\ca{T}_{\vdel}(V_I)^{d_M(V_I)}\\
&=\Directsum{I\in\mathbb{I}_{\layerV}}V_I(\vdel)^{d_M(V_I)}\\
&=\Directsum{\substack{I\in\mathbb{I}_{\layerV}\\\omega(I)\geq \delta_2}}V_I(\vdel)^{d_M(V_I)}
\oplus
\Directsum{\substack{I\in\mathbb{I}_{\layerV}\\\omega(I)< \delta_2}}V_I(\vdel)^{d_M(V_I)}.
\end{aligned}
\]

Thus $\prs{\layerV}{\big(M(\vdel)\big)}\cong
\Directsum{I\in\Iud}V_I^{d_{M(\vdel)}(V_I)}
=
\Directsum{\substack{I\in\Iud \\ \omega(I)\geq \delta_2}}V_I(\vdel)^{d_M(V_I)}
$, notice that $I$ is a dummy index on both sides. 
Now let $I\coloneqq [b_2,d]_2\sqcup[b,d_1]_1$, by comparing $V_I^{d_{M(\vdel)}(V_I)}$ with $V_J(\vdel)^{d_M(V_J)}$ for $V_J(\vdel)=V_I$, we obtain the expression of the multiplicity function $d_{M(\vdel)}$ via a change of variables:
\begin{equation}\label{eq:multiplicity-function-relation-delta}
d_{M(\vdel)}(V_{[b_2,d]_2\sqcup[b,d_1]_1})
=d_M(V_{[b_2+\delta_1+\delta_2,d+\delta_1+\delta_2]_2\sqcup[b+\delta_1,d_1+\delta_1]_1}).
\end{equation}

For $\prs{\layerV}{\iprod{b}{d}}\in\prs{\layerV}{\ca{B}}_{M(\vdel)}$, we reformulate its multiplicity as below.
% \label{eq::cPD-four-ss-vertices-eq-1}
\[
\begin{aligned}
% line 1
&\abs{\prs{\layerV}{\iprod{b}{d}}}_{M(\vdel)}
\\
=&\souwa{[b_2,d]_2\sqcup[b,d_1]_1\in \Iud}D_{M(\vdel)}\big([b_2,d]_2\sqcup[b,d_1]_1\big)
&& \text{by definition \ref{defn:unpacking-map}}
\\
% line 2
=&\souwa{[b_2,d]_2\sqcup[b,d_1]_1\in \Iud} \delta_{M(\vdel)}^{\xi^{\operatorname{ss}}}([b_2,d]_2 \sqcup [b,d_1]_1)
&& \text{definition of cPD}
\\
% line 3
=&\souwa{[b_2,d]_2\sqcup[b,d_1]_1\in \Iud} d_{M(\vdel)}(V_{[b_2,d]_2 \sqcup [b,d_1]_1})
&& \text{using theorem \ref{thm:multiplicity-from-c}}
\\
% line 4
=&\souwa{[b_2,d]_2\sqcup[b,d_1]_1\in \Iud} d_M(V_{[b_2+\delta_1+\delta_2,d+\delta_1+\delta_2]_2\sqcup[b+\delta_1,d_1+\delta_1]_1})
&& \text{applying equation (\ref{eq:multiplicity-function-relation-delta})}
\\
% line 5 change expression of summation range
=&\souwa{b_2\leq d,\ b\leq d_1} d_M(V_{[b_2+\delta_1+\delta_2,d+\delta_1+\delta_2]_2\sqcup[b+\delta_1,d_1+\delta_1]_1})
&&
\\
% line 6 
=&\souwa{b_2+\delta_1+\delta_2\leq d+\delta_1+\delta_2,\ b+\delta_1\leq d_1+\delta_1} d_M(V_{[b_2+\delta_1+\delta_2,d+\delta_1+\delta_2]_2\sqcup[b+\delta_1,d_1+\delta_1]_1})
&&
\\
% line 7
=&\souwa{[b_2+\delta_1+\delta_2,d+\delta_1+\delta_2]_2\sqcup[b+\delta_1,d_1+\delta_1]_1\in \Iud} d_M(V_{[b_2+\delta_1+\delta_2,d+\delta_1+\delta_2]_2\sqcup[b+\delta_1,d_1+\delta_1]_1})
&&
\\
% line 8
=&\souwa{[b'_2,d+\delta_1+\delta_2]_2\sqcup[b+\delta_1,d'_1]_1\in \Iud} d_M(V_{[b'_2,d+\delta_1+\delta_2]_2\sqcup[b+\delta_1,d'_1]_1})
&& \text{reindexing}
\\
% line 9
=&\souwa{[b'_2,d+\delta_1+\delta_2]_2\sqcup[b+\delta_1,d'_1]_1\in \Iud} 
D_M\big([b'_2,d+\delta_1+\delta_2]_2\sqcup[b+\delta_1,d'_1]_1\big)
&& \parbox{12em}{reverse operation using theorem \ref{thm:multiplicity-from-c} and the definition of cPD}
\\
% line 
=&\abs{\prs{\layerV}{\iprod{b+\delta_1}{d+\delta_1+\delta_2}}}_M.
\end{aligned}
\]

This shows that
$\prs{\layerV}{\ca{B}}_{M(\vdel)}$ can be matched with 
$\prs{\layerV}{\ca{B}}_M^{\delta_2}\subseteq \prs{\layerV}{\ca{B}}_M$. 
An element $\prs{\layerV}{\iprod{c}{e}}\in\prs{\layerV}{\ca{B}}_M$ is not matched if and only if $e-c<\delta_2$.
The expression for $\prs{\layerV}{\rho}$ follows naturally from the canonical matching.


Now we verify that $\vv{\rho}_M$ satisfies the definition of $\norm{\vdel}_1$-matching.
It is easy to see that we have $\Coim \rho_{\square}=\prs{\square}{\ca{B}}_{M(\vdel)}$ and $\Im  \rho_{\square}=\prs{\square}{\ca{B}}_M$ for $\square\in\set{2,1}$. 
For $\square=\layerV$, we have shown that $\Coim \rho_{\layerV}=\prs{\layerV}{\ca{B}}_{M(\vdel)}$ and 
$\Im\rho_{\layerV}=\prs{\layerV}{\ca{B}}_M=\prs{\layerV}{\ca{B}}_M^{\delta_2}$. 
Thus $\mu\big(D_{M(\vdel)}\big)\subseteq \Coim \vv{\rho}_M$
and 
$\mu\big(D_{M}\big)^{2\norm{\vdel}_1}\subseteq\mu\big(D_{M}\big)^{\delta_2}\subseteq \Im \vv{\rho}_M$.
On the other hand, 
for $\rho_{\layerV}\big(\prs{\square}{\iprod{b}{d}}\big)=\prs{\square}{\iprod{b'}{d'}}$ 
where $\square\in\set{2,1,\layerV}$, the following relationship holds:
\[
b'-\norm{\vdel}_1\leq b\leq d\leq d'+\norm{\vdel}_1,
\qquad
b-\norm{\vdel}_1\leq b'\leq d'\leq d+\norm{\vdel}_1
\]
as established by the explicit expression. This concludes the proof.

% We prove the equation case by case by classifying $I$ them using the number of essential vertices.
% Interval $I\in\Iud$ can have 2, 3, or 4 essential vertices (see figure \ref{fig:ss-essential-assignment-four-types} for illustrative examples). We are going to trace how the source-sink vertices change under the translation by $\ca{T}_{\vdel}$.
% \begin{itemize}
%     \item $\mathbf{\# E(I)=4}$
%     \item $\mathbf{\# E(I)=3}$
%     \item $\mathbf{\# E(I)=2}$
% \end{itemize}



\end{proof}
\end{lemma}
% See appendix \ref{appendix:proof-lemma-ss-vertices-tracing} for the proof of this lemma.



\begin{rmk}\label{rmk:helper-rep-thm-imt}
If $N$ is a representation in $\rep(\cln)\subseteq\rep(\clinf)$ and $\epsilon\in \mathbb{Z}_{\geq 0}$, then we use $N^{\epsilon}$ to denote the following subrepresentation of $N$:
\[
N^\epsilon_{(x,y)}\coloneqq \Im \varphi_N\Big((x-\epsilon,y)\to (x,y)\Big).
\]
where $(x,y)$ denote the coordinate of a representation and $\varphi$ is the transition morphism. The transition morphisms of $N^\epsilon$ inherit from $N$. Notice that this representation is not the same as $N(\vdel)$ as defined in definition \ref{defn:interleaving-distance}.
If we denote the unpacking map on connected persistence diagrams as 
\[
\begin{aligned}
\mu\big(\cPD(N)\big)=\big(\prs{2}{\ca{B}}_N,\prs{1}{\ca{B}}_N,\prs{\layerV}{\ca{B}}_N\big),
&\quad&\quad
\mu\big(\cPD(N^\epsilon)\big)=\big(\prs{2}{\ca{B}}_{N^\epsilon},\prs{1}{\ca{B}}_{N^\epsilon},\prs{\layerV}{\ca{B}}_{N^\epsilon}\big),\\
\end{aligned}
\]
Then it is easy to verify that
$\prs{\square}{\ca{B}}_{N^\epsilon}=\set{\prs{\square}{\iprod{c+\epsilon}{e}}|\prs{\square}{\iprod{c}{e}\in\prs{\square}{\ca{B}}_N^\epsilon\subseteq\prs{\square}{\ca{B}}_N}}$ for $\square\in\set{2,1,\layerV}$, where we recall that $\prs{\square}{\ca{B}}_N^\epsilon$ is the (multi-)set of elements in $\prs{\square}{\ca{B}}_N$ with length equal or greater than $\epsilon$.
Denote the inclusion $N^\epsilon\hookrightarrow N$ as $j_\epsilon$. 
    By definition, 
    $\chi_{j_{\epsilon}}$ 
    is a matching defined below for 
    $\square \in \set{2,1,\layerV}$.
    \[
    \begin{aligned}
    \prs{\square}{\ca{B}}_{N^\epsilon}&\to \prs{\square}{\ca{B}}_N\\
    \prs{\square}{\iprod{c+\epsilon}{e}}&\mapsto\prs{\square}{\iprod{c}{e}},
    \end{aligned}
    \]
and we can easily verify that $\Im\chi_{j_\epsilon}=
\Big(\mu\big(\cPD(N)\big)^\epsilon=\big(\prs{2}{\ca{B}}_N^\epsilon,\prs{1}{\ca{B}}_N^\epsilon,\prs{\layerV}{\ca{B}}_N^\epsilon\Big)$.
% which is equivalently with saying $\prs{\square}{\ca{B}}_{N^\epsilon}=\prs{\square}{\ca{B}}_{N}^\epsilon$ for $\square\in\set{2,1,\layerV}$.

\end{rmk}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{images/induced_matching_theorem_sandwiched_rep_in_between.jpg}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
%induced matching theorem
%theorem 6.1
With the preparations above, we can establish and prove an induced matching theorem for commutative ladders.
% in a form parallel to \cite[Theorem 6.1]{bauer2013induced}
\begin{thm}[Induced Matching Theorem]\label{thm:induced-matching-theorem}
Let $f\colon M\to N$ be a morphism between two interval-decomposable representations in $\rep(\cln)\subseteq\rep(\clinf)$ and denote the corresponding connected persistence diagrams using source-sink type assignment as $D_M\coloneqq \cPD(M)$, $D_N\coloneqq \cPD(N)$.
Morphism $f$ induces the following matching for $\square \in \set{2,1,\layerV}$.
\[
\begin{aligned}
\chi_f\colon \mu\big(D_M\big)\ni\prs{\square}{\ca{B}}_M&\to \prs{\square}{\ca{B}}_N\in\mu\big(D_N\big)\\
\prs{\square}{\iprod{b}{d}}&\mapsto\prs{\square}{\iprod{b'}{d'}}.
\end{aligned}
\]
Let $\vec{\delta}=(\delta_1,\delta_2)$ be a tuple in $\mathbb{Z}^2_{\geq 0}$, and define $\epsilon\coloneqq\norm{\vdel}_{1}=\delta_1+\delta_2$.
Then
\begin{enumerate}
    \item $b'\leq b\leq d'\leq d$.
    \item If $\Coker f$ is $\vdel$-trivial, then $\mu(D_N)^{\epsilon}\subseteq \Im\chi_f$ and 
    \[
    b'\leq b\leq b'+\epsilon.
    \]
    \item Dually, if $\Ker f$ is $\vdel$-trivial, then $\mu(D_M)^{\epsilon}\subseteq \Coim\chi_f$ and
    \[
    d-\epsilon\leq d'\leq d.
    \]
\end{enumerate}


\begin{proof}
\hfill
\begin{enumerate}
    \item Statement 1 is exactly proposition \ref{prop:relations-between-births-and-deaths}.
    \item 
    We keep using the auxiliary representations defined in remark \ref{rmk:helper-rep-thm-imt}.
    Entries in the tuples can be written as $\mu(D_N)^\epsilon=\big(\prs{2}{\ca{B}}_N^\epsilon,\prs{1}{\ca{B}}_N^\epsilon,\prs{\layerV}{\ca{B}}_N^\epsilon\big)$
    and $\Im\chi_f=\big(\prs{2}{\ca{B}}_{\Im f},\prs{1}{\ca{B}}_{\Im f},\prs{\layerV}{\ca{B}}_{\Im f}\big)\subseteq \mu\big(D_N\big)$.
    %The strategy would be to sandwich $\prs{\square}{\ca{B}}_{\Im f}$ between $\prs{\square}{\ca{B}}_{N^\epsilon}$ and $\prs{\square}{\ca{B}}_N$. 
    First, we use the following commutative diagram to show that $N^\epsilon\subseteq \Im f$.
    Arrows involved in the proof are highlighted at both layers and only labeled in the second layer for readability.
    \[
    \begin{tikzcd}[row sep=scriptsize, column sep=normal]
    %layer 6 (upper)
    & & (\Coker f)_{(x-\epsilon,2)}  \arrow[rrr,"\varphi_{\Coker f}",color=blue] \arrow[from=ddd] & & & (\Coker f)_{(x,2)} \arrow[from=ddd] \\
    %layer 5 (upper)
    & N_{(x-\epsilon,2)} \arrow[ur,"\coker f",color=blue] \arrow[rrr,crossing over,"\varphi_N"',color=blue] \arrow[from=ddd] &  & & N_{(x,2)} \arrow[ur,"\coker f"',color=blue]\\
    %layer 4 (upper)
    M_{(x-\epsilon,2)} \arrow[ur]\arrow[rrr, crossing over] \arrow[from=ddd,crossing over] & & & M_{(x,2)}\arrow[ur]\\
    %layer 3 (lower)
    & & (\Coker f)_{(x-\epsilon,1)} \arrow[rrr,color=blue] & & &(\Coker f)_{(x,1)} \\
    %layer 2 (lower)
    & N_{(x-\epsilon,1)} \arrow[ur,color=blue] \arrow[rrr,color=blue] & & & N_{(x,1)} \arrow[ur,color=blue] \arrow[uuu, crossing over] \\
    %layer 1 (lower)
    M_{(x-\epsilon,1)} \arrow[rrr] \arrow[ur]& & & M_{(x,1)} \arrow[ur] \arrow[uuu, crossing over] \\
    \end{tikzcd}.
    \]
By commutativity, for $x\in\mathbb{Z}$ and $y=1,2$ we have
\begin{equation}\label{eq:imt-proof-eq1}
\coker f\circ \varphi_N\big((x-\epsilon,y)\to(x,y)\big)=\varphi_{\Coker f}\big((x-\epsilon,y)\to(x,y)\big)\circ\coker f
\end{equation}
Since $\Coker f$ is $\vdel$-trivial, the natural morphism $\Coker f\to (\Coker f)(\vdel)$ vanishes. Specifically, the following two families of maps  vanish:
\begin{itemize}
    \item $\varphi_{\Coker f}\big((x,2)\to (x+\delta_2+\delta_1,2)\big)$;
    \item $\varphi_{\Coker f}\big((x,1)\to (x+\delta_1,1)\big)$.
\end{itemize}
Thus equation (\ref{eq:imt-proof-eq1}) vanishes as well by choice of $\epsilon$. From that we deduce 
${\Im f\supseteq \varphi_N\big((x-\epsilon,y)\to(x,y)\big)=N^\epsilon}$.
We have proved that the following diagram commutes:
\[
\begin{tikzcd}[column sep=large]
    & N  \\
    N^\epsilon \arrow[ur,hookrightarrow,"j_\epsilon"]\arrow[dr,hookrightarrow,"j"'] & \\
    & \Im f\arrow[uu,hookrightarrow,"j_f"'],
\end{tikzcd}
\]
so by proposition \ref{prop:partial_functorial_induced_matching}, $\chi_{j_\epsilon}=\chi_{j_f}\circ\chi_j$.
On the other hand, by definition $\chi_f=\chi_{j_f}\circ\chi_{q_f}$ by factorizing $f$ as 
$\begin{tikzcd}[column sep=small]
M \arrow[r,two heads,"q_f"] &\Im f \arrow[r,hook,"j_f"] & N
\end{tikzcd}$.
Thus $\Im\chi_{j_\epsilon}\subseteq \Im\chi_{j_f}=\Im\chi_f$, and by remark \ref{rmk:helper-rep-thm-imt} $\prs{\square}{\ca{B}}_{N^\epsilon}\subseteq\prs{\square}{\ca{B}}_{\Im f}\subseteq \prs{\square}{\ca{B}}_{N}$ for $\square\in\set{2,1,\layerV}$. 
% The other inclusion $\prs{\square}{\ca{B}}_{\Im f}\subseteq \prs{\square}{\ca{B}}_{N}$ is obvious since $\Im f\subseteq N$.

For the inequality, it suffices to prove that $b\leq b'+\epsilon$ as the left half coming from the first statement.
Since $\big(\prs{2}{\ca{B}}_N^\epsilon,\prs{1}{\ca{B}}_N^\epsilon,\prs{\layerV}{\ca{B}}_N^\epsilon\Big)=\Im \chi_{j_\epsilon}\subseteq\chi_{\Im f}$,
there are two possibilities for $\prs{\square}{\iprod{b'}{d'}}$:
\begin{itemize}
\item  $\prs{\square}{\iprod{b'}{d'}}\notin \prs{\square}{\ca{B}}_N^\epsilon$: then by definition $d'-b'\leq \epsilon$, combining with statement 1 yields $b\leq b'+\epsilon$.
\item  $\prs{\square}{\iprod{b'}{d'}}\in \prs{\square}{\ca{B}}_N^\epsilon$: this element is in the image of $\Im \chi_{j_\epsilon}$, 
then by remark \ref{rmk:helper-rep-thm-imt}, 
$\prs{\square}{\iprod{b'}{d'}}=\chi_{j_\epsilon}\big(\prs{\square}{\iprod{b'+\epsilon}{d'}}\big)
=\chi_{j_f}\circ\chi_j\big(\prs{\square}{\iprod{b'+\epsilon}{d'}}\big)$. 
On the other hand, by assumption we have $\chi_f\big(\prs{\square}{\iprod{b}{d}}\big)=\chi_{j_f}\circ\chi_{q_f}\big(\prs{\square}{\iprod{b}{d}}\big)
=\chi_{j_f}\big(\prs{\square}{\iprod{b}{d'}}\big)$. 
As $\chi_{j_f}$ is injective, we obtain that $\chi_j\big(\prs{\square}{\iprod{b'+\epsilon}{d'}}\big)=\prs{\square}{\iprod{b}{d'}}$,
from which we conclude that $b\leq b'+\epsilon$ by proposition \ref{prop:relations-between-births-and-deaths}.
\end{itemize}
\item For proving the dual statement, first we notice that the map $q_f$ in $\begin{tikzcd}[column sep=small]
M \arrow[r,two heads,"q_f"] &\Im f \arrow[r,hook,"j_f"] & N
\end{tikzcd}$
induces a map $\tilde{q}$ (which is an isomorphism) starting from $\Coim f=M/\Ker f$ as in the following commutative diagram.
\begin{equation}\label{eq:imt-cd-diagram-2}
\begin{tikzcd}
\Ker f\arrow[r,hook,"\ker f"]&M\arrow[r,two heads,"q_f"]\arrow[d,two heads,"\coim f"']&\Im f\arrow[r,hook,"j_f"]& N\\
&M/\Ker f \arrow[ur,two heads,"\tilde{q}_f"']& &
\end{tikzcd}
\end{equation}
It is easy to see that $\tilde{q}_f$ is well-defined and still surjective. So by proposition \ref{prop:partial_functorial_induced_matching},
we obtain $\chi_{q_f}=\chi_{\tilde{q}_f}\circ\chi_{\coim f}$. Thus $\chi_f=\chi_{j_f}\circ\chi_{q_f}=\chi_{j_f}\circ\chi_{\tilde{q}_f}\circ\chi_{\coim f}$ and 
\begin{equation}\label{eq:imt-surj-intermediate-2}
\Coim \chi_f=\Coim \chi_{\coim f}.
\end{equation}
Define an auxiliary subrepresentation of $M$:
\[
M^{< \epsilon}_{(x,y)}\coloneqq \Ker \varphi_M\Big((x-(\epsilon-1),y)\to (x,y)\Big).
\]
It is easy to verify that 
$\prs{\square}{\ca{B}}_{M^{<\epsilon}}=
\set{\prs{\square}{\iprod{c}{e}}|\prs{\square}{\iprod{c}{e}}\in\prs{\square}{\ca{B}}_M\mbox{ and }e-c<\epsilon}$
simply by using the definition.
Considering the quotient representation $Q\coloneqq M/M^{<\epsilon}$, we see that all intervals with lengths shorter than $\epsilon$ are nullified. Set $D_Q\coloneqq \cPD(Q)$, applying the unpacking map to this connected persistence diagram yields
\[
\mu(D_Q)\ni\prs{\square}{\ca{B}}_{Q}=\set{\prs{\square}{\iprod{c}{e}}|\prs{\square}{\iprod{c}{e}}\in\prs{\square}{\ca{B}}_M\mbox{ and }e-c\geq\epsilon}.
\]
Notice that $\mu(D_Q)=\mu(D_M)^\epsilon$, which is what we need in the statement. 
The surjective map ${\pi\colon M\to Q}$ induces a matching between from $\mu\big(D_M\big)$ to $\mu\big(D_Q\big)$. By the constructing definition of $\chi_\pi$, it is easy to see that $\Coim \chi_\pi=\mu(D_M)^\epsilon\subseteq\mu(D_M)$.
To obtain the desired inclusion relationship, consider the following commutative diagram:
\[
\begin{tikzcd}
    M\arrow[r,two heads,"\coim f"]\arrow[d,two heads,"\pi"']&M/\Ker f\arrow[ld,two heads,"\theta"]\\
    Q%M/M^{<\epsilon}.
\end{tikzcd}.
\]
We claim that $\Ker f\subseteq M^{<\epsilon}$ so $\theta$ is well-defined. Then by proposition \ref{prop:partial_functorial_induced_matching}
$\chi_\pi=\chi_\psi\circ\chi_{\coim f}$, thus $\Coim \chi_{\coim f}\supseteq\Coim \chi_\pi=\mu\big(D_M\big)^\epsilon$.
Combining with equation (\ref{eq:imt-surj-intermediate-2}) yields $\mu(D_M)^{\epsilon}\subseteq \Coim\chi_f$.

Now we prove the claim $\Ker f\subseteq M^{<\epsilon}$. This inclusion relationship can be read out from the commutative diagram below.
As in the previous case, we highlight morphisms used and label them in the second layer
\[
    \begin{tikzcd}[row sep=scriptsize, column sep=normal]
    %layer 6 (upper)
    & & N_{(x-\epsilon,2)}  \arrow[rrr,crossing over] \arrow[from=ddd] & & & N_{(x,2)} \arrow[from=ddd] \\
    %layer 5 (upper)
    & M_{(x-\epsilon,2)} \arrow[ur] \arrow[rrr,crossing over,"\varphi_M",color=blue] \arrow[from=ddd] &  & & M_{(x,2)} \arrow[ur]\\
    %layer 4 (upper)
    (\Ker f)_{(x-\epsilon,2)} \arrow[ur,color=blue,"\ker f"]\arrow[rrr, crossing over,color=blue,"\varphi_{\Ker f}"'] \arrow[from=ddd,crossing over] & & & (\Ker f)_{(x,2)}\arrow[ur,color=blue,"\ker f"']\\
    %layer 3 (lower)
    & & N_{(x-\epsilon,1)} \arrow[rrr] & & &N_{(x,1)} \\
    %layer 2 (lower)
    & M_{(x-\epsilon,1)} \arrow[ur] \arrow[rrr,color=blue] & & & M_{(x,1)} \arrow[ur] \arrow[uuu, crossing over] \\
    %layer 1 (lower)
    (\Ker f)_{(x-\epsilon,1)} \arrow[rrr,color=blue] \arrow[ur,color=blue]& & & (\Ker f)_{(x,1)} \arrow[ur,color=blue] \arrow[uuu, crossing over] \\
    \end{tikzcd}.
    \]
Using commutative relations, for $x\in\mathbb{Z}$ and $y=1,2$
\begin{equation}\label{eq:imt-proof-eq3}
\varphi_M\big((x-\epsilon,y)\to(x,y)\big)\circ\ker f = \ker f\circ \varphi_{\Ker f}\big((x-\epsilon,y)\to(x,y)\big).
\end{equation}
As $\Ker f$ is $\vdel$-trivial, following similar steps as in the previous case, we can show that $\varphi_{\Ker f}\big((x-\epsilon,y)\to(x,y)\big)$ vanishes. Thus $\varphi_M\big((x-\epsilon,y)\to(x,y)\big)\circ\ker f=0$ and it follows that ${(\Ker f)_{(x,y)}\subseteq \Ker \varphi_M\big((x-\epsilon,y)\to(x,y)\big)=M^{<\epsilon}_{(x,y)}}$, finishing the proof of the inclusion relationship.

For the inequality, it suffices to prove that $d-\epsilon\leq d'$. Let $\prs{\square}{\iprod{b}{d}}$ be an element in $\Coim \chi_f$. 
Likewise, there are two possibilities for it.
\begin{itemize}
    \item $\prs{\square}{\iprod{b}{d}}\notin \prs{\square}{\ca{B}}_M^\epsilon$: then $d-b<\epsilon$. Using $b\leq d'$ we get $d-\epsilon\leq d'$.
    \item $\prs{\square}{\iprod{b}{d}}\in \prs{\square}{\ca{B}}_M^\epsilon$: then $\prs{\square}{\iprod{b}{d}}\in\Coim \chi_\pi$. 
    By definition $\chi_{\pi}(\prs{\square}{\iprod{b}{d}})=\prs{\square}{\iprod{b}{d}}=\chi_\theta\circ\chi_{\coim f}(\prs{\square}{\iprod{b}{d}})$.
    Notice that both $\chi_\theta$ and $\chi_{\coim f}$ matches an element of form $\prs{\square}{\iprod{c}{e}}$ to another element of form $\prs{\square}{\iprod{c}{e'}}$ with $e'<e$ as $\theta$ and $\coim f$ are surjective, 
    so $\chi_{\coim f}(\prs{\square}{\iprod{b}{d}})=\prs{\square}{\iprod{b}{d}}$. 
    Now we turn back to commutative diagram (\ref{eq:imt-cd-diagram-2}), and notice that 
    \[
    \begin{aligned}
    \chi_f\big(\prs{\square}{\iprod{b}{d}}\big)&=\chi_{j_f}\circ\chi_{q_f}\big(\prs{\square}{\iprod{b}{d}}\big)\\
    &=\chi_{j_f}\circ\chi_{\tilde{q}_f}\circ\chi_{\coim f}\big(\prs{\square}{\iprod{b}{d}}\big)\\
    &=\chi_{j_f}\circ\chi_{\tilde{q}_f}\big(\prs{\square}{\iprod{b}{d}}\big)\\
    &=\prs{\square}{\iprod{b'}{d'}}
    \end{aligned}
    \]
    The map $\tilde{q}_f$ is an isomorphism, so as a tuple of multisets $\mu\big(\cPD(\Im f)\big)$ and $\mu\big(\cPD(M/\Ker f)\big)$ are identical, which means the induced matching $\chi_{\tilde{q}_f}$ leaves all elements invariant. Matching $\chi_{j_f}$ will only change the birth index. In a conclusion, we get $d'=d$, which satisfies the inequality.
\end{itemize}
\end{enumerate}
\end{proof}
\end{thm}



% Assume that $\Ker f$ and $\Coker f$ are $2\vec{\delta}$-trivial.
% Then we have a $\vec{\delta}$-matching
% \[
% \mu(f)\circ r_M^{\vec{\delta}}
% \colon
% \mu\Big(\cPD\big(M(\vec{\delta})\big)\Big)
% \centernot\rightarrow
% \mu(\big(\cPD(N)\big).
% \]

%lemma6.3
\begin{lemma}
If $M$ and $N$ in $\rep(\cln)\subseteq\rep(\clinf)$ are $\vdel$-interleaved with $f\colon M\to N(\vdel)$
being an interleaving morphism, then $\Ker f$ and $\Coker f$ are $2\vdel$-trivial.
\begin{proof}
The following commutative diagram can be formulated using the definition of $\vdel$-interleaving.
\[
\begin{tikzcd}[row sep=normal, column sep=small]
\Ker f\arrow[r, from=1-1, to=1-3,"\psi"]\arrow[rd,"\iota"'] & & \Ker [f(2\vdel)]\arrow[rd,"\iota^{2\vdel}"]& &   \\
  & M\arrow[rr,"\varphi_M^{2\vdel}"]\arrow[rd,"f"']& & M(2\vdel)\arrow[rd,"f(2\vdel)"]&   \\
  &  & N(\vdel)\arrow[rr]\arrow[ru,"g(\vdel)"] &  & N(3\vdel) \\
\end{tikzcd}
\]
It can be verified directly that $\Ker[f(2\vdel)]=[\Ker f](2\vdel)$, so it suffices to show that $\psi=0$,
which is equivalent with $\iota^{2\vdel}\circ \psi$, as $\iota^{2\vdel}$ is injective. 
Commutative relations allow us to conclude that
${\iota^{2\vdel}\circ \psi=\varphi_M^{2\vdel}\circ \iota=g(\vdel)\circ f\circ\iota=0}$.
This proves that $\Ker f$ is $2\vdel$-trivial. The dual statement can be shown using similar reasoning.
\end{proof}
\end{lemma}

Finally, we state the algebraic stability theorem for interval-decomposable representations of commutative ladders, as a corollary of the induced matching theorem
%theorem 6.4 explicit formulation of algebraic stability
\begin{thm}[Algebraic Stability Theorem]
If $M$ and $N$ are interval-decomposable representations in $\rep(\cln)\subseteq\rep(\clinf)$
and ${f\colon M\to N(\vdel)}$ is a $\vdel$-interleaving morphism. 
Denote their connected persistence diagrams by $D_M\coloneqq \cPD(M)$ and $D_N\coloneqq \cPD(N)$.
Then 
${\vv{\rho}_N\circ \ca{X}_f\colon \mu(D_M)\centernot\rightarrow\mu(D_N)}$ 
is a $(\norm{\vdel}_{1}+\delta_2)$-matching.
In particular, 
\[
d_B(D_M,D_N)\leq 
2\cdot d_I(M,N).
\]
\begin{proof}
First, we prove the inclusion relationship involved in the definition of $(\norm{\vdel}_{1}+\delta_2)$-matching.
By the previous lemma, $\Ker f$ and $\Coker f$ are both $2\vdel$-trivial.
Using theorem \ref{thm:induced-matching-theorem}, we have
$\mu(D_M)^{2\norm{\vdel}_1}\subseteq\Coim \chi_f$.
From the proof of lemma \ref{lemma:cPD-four-ss-vertices}, we have
$\Coim \vv{\rho}_N=\mu(D_{N(\vdel)})$, thus ${\mu(D_M)^{2\norm{\vdel}_1}\subseteq\Coim(\vv{\rho}_N\circ\chi_f)}$ as well,
which is stronger than the required condition $\mu(D_M)^{2(\norm{\vdel}_{1}+\delta_2)}\subseteq\Coim(\vv{\rho}_N\circ\chi_f)$.
Similarly, from $\mu(D_{N(\vdel)})^{2\norm{\vdel}_1}\subseteq \Im \chi_f$ and the explicit expression of $\vv{\rho}_N$,
we have $\mu(D_N)^{2\norm{\vdel}_1+\delta_2}\subseteq\Im(\vv{\rho}_N\circ\chi_f)$,
which is also stronger than the required condition $\mu(D_N)^{2(\norm{\vdel}_1+\delta_2)}\subseteq\Im(\vv{\rho}_N\circ\chi_f)$.

To verify the inequalities involved in the composited matching, consider the following maps.
Inequalities obtained from 
theorem \ref{thm:induced-matching-theorem} and lemma \ref{lemma:cPD-four-ss-vertices}
are written under the matched elements.
\begin{equation}
\begin{tikzcd}[column sep=5.4em,ampersand replacement=\&]
\mu(D_M)\arrow[r,"\chi_f"]\&\mu(D_{N(\vdel)})\arrow[r,"\vv{\rho}_N"]\&\mu(D_N)\\
\prs{\square}{\iprod{b}{d}}\arrow[r,mapsto]\&\prs{\square}{\iprod{b'}{d'}}\arrow[r,mapsto]\&\prs{\square}{\iprod{b''}{d''}}\\
\&
\begin{aligned}
b'&\leq b&&\leq b'+2\norm{\vdel}_{1},\\
d-2\norm{\vdel}_{1}&\leq d'&&\leq d\\
\\
\\
\\
\end{aligned} 
\&
\begin{aligned}
% 2
\square=2
&\colon
\begin{cases}
b''=b'+\delta_1+\delta_2
\\
d''=d'+\delta_1+\delta_2
\end{cases}\\
% 1
\square=1
&\colon
\begin{cases}
b''=b'+\delta_1
\\
d''=d'+\delta_1
\end{cases}\\
%2/1
\square=\layerV
&\colon
\begin{cases}
b''=b'+\delta_1
\\
d''=d'+\delta_1+\delta_2
\end{cases}
\end{aligned}
\\
\end{tikzcd}
\end{equation}

These inequalities can be reduced to the forms below by canceling $b'$ and $d'$.
\[
\begin{aligned}
%2
\square=2&\colon 
\left\{ 
\begin{array}{llll}
         b''-\delta_1-\delta_2 & \leq b & \leq d & \leq d''+\delta_1+\delta_2\\
        b-\delta_1-\delta_2 & \leq b'' & \leq d'' & \leq d+\delta_1+\delta_2\\
\end{array},
\right.
\\
%1
\square=1&\colon 
\left\{ 
\begin{array}{llll}
        b''-\delta_1 & \leq b & \leq d & \leq d''+\delta_1+2\delta_2\\
        b-\delta_1-2\delta_2 & \leq b'' & \leq d'' & \leq d+\delta_1\\
\end{array},
\right.
\\
%2/1
\square=\layerV&\colon 
\left\{ 
\begin{array}{llll}
        b''-\delta_1 & \leq b & \leq d & \leq d''+\delta_1+\delta_2\\
        b-\delta_1-2\delta_2 & \leq b'' & \leq d'' & \leq d+\delta_1+\delta_2\\
\end{array},
\right.
\\
\end{aligned}
\]
All the inequalities are the same or stronger than what is needed for $\vv{\rho}_N\circ \chi_f$ being a ${\norm{\vdel}_1+\delta_2}$-matching, finishing the verification.

For the last inequality in the statement, 
suppose $d_I(M,N)=\epsilon$, then by definition, there exists $\vdel$ with $\norm{\vdel}_1=\epsilon$ (the infimum can always be reached as the norm takes value in $\mathbb{Z}$, which is discrete). 
Then from what we just proved, there exists a $\norm{\vdel}_1+\delta_2$-matching between $D_M$ and $D_N$,
so by the definition of bottleneck distance $d_B(D_M,D_N)\leq \norm{\vdel}_1+\delta_2\leq 2\norm{\vdel}_1=2\epsilon$, concluding the proof.
\end{proof}
\end{thm}
% postscript:
% maybe we want to remove the extra $+\delta_2$ in the statement, 
% that requires a change in theorem 5.29, specifically
% for layer 2: $b'\leq b\leq'+2\norm{\vdel}_1$, $d-2\norm{\vdel}_1\leq d'\leq d$
% for layer 1: $b'\leq b+\delta_2$, $b+\delta_2\leq b'+2\norm{\vdel}_1$,
% for layer 2/1: $b'\leq b+\delta_2\leq b'+2\norm{\vdel}_1$, $d-2\norm{\vdel}_1\leq d'\leq d$


% \colorbox{red}{distance between lines, $[b_1,d_1]_1\sqcup[b_2,-]_2$}

% \begin{itemize}
%     \item Commutative ladder module $\rep(\cln)$ $\Rightarrow$
%     \item $\xi$-compressed multiplicities $\Rightarrow$
%     \item connected persistence diagrams
% \end{itemize}
% \vspace{10pt}
% Need to define the following two distances (pseudo-metric):
% \begin{itemize}
%     \item interleaving distance on $\rep(\cln)$
%     \item bottleneck distance on cPDs.
% \end{itemize}
% \vspace{10pt}
% Using the language of \textit{Theory of interleavings on categories with a flow} (see Definition 2.1 and Definition 3.1)

% \begin{defn}
% Settings
% \begin{itemize}
%     \item $\mathcal{P}\coloneqq \mathbb{R}\times \mathbb{F}_2$
%     \item $\mathcal{D}=\cat{Vect}_\Bbbk$
% \end{itemize}
% A commutative ladder module is a function $M\in \mathcal{D}^{\mathcal{P}}$ (or $\rep_{\mathbb{k}}(\mathcal{P})$)
% such that for any $(1,a),(1,b),(0,a),(0,b)$ with $a<b$, the corresponding square commutes.
% \vspace{10pt}
% We can define two kinds of flows on $\mathcal{P}$ (\textit{i.e.}, two families of endofunctors on $\mathcal{P}$.
% Let $\varepsilon\in [0,\infty)$
% \begin{enumerate}
%     \item overall shift functor $\mathcal{T}_{\varepsilon}$;
%     \item upper dislocation functor $\mathcal{U}_{\varepsilon}$;
%     %\item lower dislocation functor $\mathcal{L}_{\varepsilon}$; not a poset morphism
% \end{enumerate}
% \end{defn}
% \vspace{100pt}
% \begin{defn}
% Two modules (functors/representations) $\mathbf{F}$ and $\mathbf{G}$ are said to be $\vec{\varepsilon}$-interleaved if there exist a pair of natural transformations 
% $\varphi\colon \mathbf{F}\Rightarrow \mathbf{G}\Omega_{\vec{\varepsilon}}$ and 
% $\psi\colon \mathbf{G}\Rightarrow \mathbf{F}\Omega_{\vec{\varepsilon}}$ 
% such that the diagrams below commute.
% \vspace{70pt}
% We have
% \begin{itemize}
%     \item $\vec{\varepsilon}=(\varepsilon_1,\varepsilon_2)$;
%     \item $\Omega_{\vec{\varepsilon}}=\mathcal{T}_{\varepsilon_1}\circ \mathcal{U}_{\varepsilon_2}$.
% \end{itemize}
% The interleaving distance with respect to $\Omega_{\vec{\varepsilon}}$ is 
% \[
% d_{\Omega}(\mathbf{F},\mathbf{G})
% =\inf\set{\norm{\vec{\varepsilon}}_{\infty}|
% \text{
% $\mathbf{F}$ and $\mathbf{G}$ are $\vec{\varepsilon}$-interleaved
% }
% }.
% \]
% \end{defn}

% \vspace{20pt}

% \subsubsection{Barcodes and bottleneck distance}

% Let $\mathbf{M}$ be a commutative ladder module.
% \[
% \mathcal{B}(\mathbf{M})\coloneqq
% \set{\big(I,c_M^\xi(V_I)\big)}_{I\in\mathbb{I}}
% \]
% is a multiset.

% Define the bottleneck distance:
% \[
% d_B(\mathcal{\mathbf{F}},\mathcal{\mathbf{G}})
% =\inf\set{
% \norm{\vec{\varepsilon}}_{\infty}
% |
% \exists \text{ an $\vec{\varepsilon}$-matching between 
% $\mathcal{\mathbf{F}}$ and $\mathcal{\mathbf{G}}$.}
% }
% \]
% \newpage



==> legacy/obsolete.tex <==
\begin{multicols}{3}
\begin{itemize}
    \item $1 \Leftrightarrow\ 20$
    \item $2 \Leftrightarrow\ 19$
    \item $3 \Leftrightarrow\ 18$
    \item $4 \Leftrightarrow\ 17$
    \item $5\ \Leftrightarrow\ 14$
    \item $6\ \Leftrightarrow\ 13$
    \item $7\ \Leftrightarrow\ 8$
    \item $8\ \Leftrightarrow\ 7$
    \item $9\ \Leftrightarrow\ $
    \item $N_{10}\ \Leftrightarrow\ N_{12}$
    \item $N_{11}\  \rotatebox[origin=c]{90}{$\circlearrowleft$}$
\end{itemize}
\end{multicols}





\subsubsection{Intervals whose multiplicity can be solved directly}

By equation \ref{eq:delta-mult-1}, for a fixed boundary compression method $*$ and a fixed $I$, if $\delta_N^{*}(I)$ for all $N\in\mathcal{N}$, then $d_M(I)=\delta^*_M(I)$. 





There are 46 intervals from which $d_M(I)$ can be solved directly since $\delta_N^*(I)$ for all $N\in\mathcal{N}$, where * is ss or zz. 


We split $\mathcal{I}$ into the following two sets:
\begin{itemize}
        \item $\mathcal{I}^s$: set of intervals with $d_M(I)$ already solved;
        \item $\mathcal{I}^u$: set of intervals with $d_M(I)$ remains unsolved.
\end{itemize}

We are then left with 
\begin{itemize}
    \item 18 equations (9 form each method), where we know at most 17 of them are linearly independent since $\delta^{ss}_{N_7}=\delta^{zz}_{N_7}$
\end{itemize}
to solve
\begin{itemize}
    \item In total 30 unknowns:
    \item $d_M(N_1),\ \cdots, d_M(N_{21})$ %(number is reduced by using the symmetric operation from section one);
    \item $d_M(J_1),\ \cdots, d_M(J_9)$ for $J_i\in \mathcal{I}^u$.
\end{itemize}

Notice that the $c$ maps from both compression methods yield the same value for $M_7$. So new boundary compression method is needed in order to solve this system. We need a new map $c^*_M$ such that it satisfies the lemmas in note \textit{2020-08-18(境界圧縮について)}.

With the goal of distinguishing $M_7$ in mind, and noticing that we do not have to consider about modifying the compression of zigzag-shaped intervals. we tried almost all possibilities. But none of them gives us new a new result.

We can try to define a new boundary compression method if violating lemma 3 in the note is allowed. Then equation (\ref{eq:delta-mult-1}) will become the following form:

\begin{equation}\label{eq:delta-mult-2}
\begin{aligned}
\delta_M^*(I)&=\souwa{L\in\mathcal{L}}d_M(L)\cdot \delta^*_L(I)\\
&=\souwa{N\in\mathcal{N}}d_M(N)\cdot \delta^*_N(I) + \souwa{J\in\mathcal{I}}d_M(J)\cdot \delta^*_J(I)\\
&=\souwa{N\in\mathcal{N}}\delta^*_N(I)\cdot d_M(N) + \souwa{J\in\mathcal{I}^u}d_M(J)\cdot \delta^*_J(I)+ \souwa{J\in\mathcal{I}^s}d_M(J)\cdot \delta^*_J(I)\\
&=\souwa{N\in\mathcal{N}}\delta^*_N(I)\cdot d_M(N) + \souwa{J\in\mathcal{I}^u}d_M(J)\cdot \delta^*_J(I)+ \souwa{J\in\mathcal{I}^s}\delta^{*(J)}_M(J)\cdot \delta^*_J(I).\\
\end{aligned}
\end{equation}

Set $\mathcal{I}^u=\set{I_1,\cdots,I_p}$, these set of equations can be expressed in matrix form:
\begin{equation}
\begin{aligned}
&
\begin{pmatrix}
\delta_{N_1}^*(I_1)&\delta_{N_2}^*(I_1)&\cdots&\delta_{N_q}^*(I_1)&\delta_{I_1}^*(I_1)&\delta_{I_2}^*(I_1)&\cdots &\delta_{I_p}^*(I_1)\\
\delta_{N_1}^*(I_2)&\ddots&\cdots&\delta_{N_q}^*(I_2)&\delta_{I_1}^*(I_2)&\ddots&\cdots &\delta_{I_p}^*(I_2)\\
\vdots&\vdots&\ddots&\vdots&\vdots&\vdots&\ddots& 0\\
\delta_{N_1}^*(I_p)&\cdots&\cdots&\delta_{N_q}^*(I_p)&\delta_{I_1}^*(I_p)&\cdots&\cdots &\delta_{I_p}^*(I_p)\\
\end{pmatrix}
\begin{pmatrix}
d_M(N_1)\\
\vdots\\
d_M(N_q)\\
d_M(I_1)\\
\vdots\\
d_M(I_p)\\
\end{pmatrix}
\\
=&
\begin{pmatrix}
\delta_M^*(I_1)-\souwa{J\in\mathcal{I}^s}\delta^{*(J)}_M(J)\cdot \delta^*_J(I_1)\\
\delta_M^*(I_2)-\souwa{J\in\mathcal{I}^s}\delta^{*(J)}_M(J)\cdot \delta^*_J(I_2)\\
\vdots\\
\delta_M^*(I_p)-\souwa{J\in\mathcal{I}^s}\delta^{*(J)}_M(J)\cdot \delta^*_J(I_p)\\
\end{pmatrix}
\end{aligned}
\end{equation}

Slides content
\begin{itemize}
    \item Matrix formulation
    \item rank via ss and zg
    \item the new compression method
    \item release the conditions
    \item computational workflow
\end{itemize}

==> sec3/main_lemma_original_proof.tex <==
\begin{lemma}\label{lemma:rank-invariant-lemma-2}
    With the same settings as in the previous lemma
    and let $M$ be a representation of $G$. 
    Then the following equation holds:
    \[
        c^{\xi}_M(V_B)=\rank\big(M(\alpha_l)\cdots M(\alpha_1)\big).
    \]
    \begin{proof}
        We introduce the following restrictions of representations and essential assignment:
        \begin{itemize}
            \item restrict the representation $M\in\rep(G)$ to $\restr{M}{B}\in\rep(B)$;
            \item restrict the representation $V_B\in \mathcal{I}_{\rep(G)} \subseteq \rep(G)$ to $\restr{V_B}{B}\in\mathcal{I}_{\rep(B)}\subseteq \rep(B)$, denoted as $\lozenge_B$
            \item restrict the essential assignment $\xi\colon \IG\to\courses(G)$ 
        to $\widetilde{\xi}\colon\mathbb{I}_B\to \courses(B)$.
        \end{itemize}
        With these preparations, 
        we rewrite the $\xi$-compressed multiplicity on the left-hand side as follows:
        \begin{equation}\label{eq:compression-to-restricted-compression}
        c^{\xi}_M(V_B)
        =
        d_{\tour_{\xi(B)}(M)}\big[\tour_{\xi(B)}(V_{B})\big]
        =
        d_{\tour_{\widetilde{\xi}(B)}(\restr{M}{B})}\big[\tour_{\widetilde{\xi}(B)}(\restr{V_{B}}{B})\big]
        =
        c^{\widetilde{\xi}}_{\restr{M}{B}}(\lozenge_B).
        \end{equation}
        % \end{equation}

        Now we show that the $\widetilde{\xi}$-compressed multiplicity above is equal to $r\coloneqq\rank\big(M(p)\big)\coloneqq\rank\big(M(\alpha_l)\cdots M(\alpha_1)\big)$.
        
        It is easy to verify that $\lozenge_B$ is an indecomposable projective-injective representation.
        % notice that \operatorname{soc}(\lozenge_B)\cong S(t) (the simple representation associated with t)
        % by the argument in Lemma 2.2 of Elements of the Representation Theory of Associative Algebras.pdf.
        Therefore, we can apply \cite[Theorem 31]{asashiba2017decomposition} 
        and the remark below it, which yields the following equations:
        % hom are quotient algebra homs
        % see Lemma 2.2 associative algebras for computation of socle
        \[
        \begin{aligned}
        d_{\restr{M}{B}}(\lozenge_B)&=\dim_{\Bbbk} \Hom(\lozenge_B,\restr{M}{B})
        -
        \dim_{\Bbbk}\Hom\left(\lozenge_B/\operatorname{soc}(\lozenge_B),\restr{M}{B}\right)\\
        &=\dim_{\Bbbk}M(s)-\big(\dim_{\Bbbk}M(s)-\rank(M(p))\big)\\
        &=\rank(M(p))\\
        &= r.
        \end{aligned}
        \]
        %
        Thus $\restr{M}{B}$ can be written as a direct sum ${\restr{M}{B}=\lozenge_B^{\oplus r}\oplus N}$, with $N\in\rep(B)$ not having $\lozenge_B$ as a direct summand. 
        %
        Apply the additivity (Proposition \ref{prop:compression-additive}) to this decomposition, 
        we have
        \[
        c^{\widetilde{\xi}}_{\restr{M}{B}}(\lozenge_B)
        =
        c^{\widetilde{\xi}}_{\lozenge_B^{\oplus r}\oplus N}(\lozenge_B)
        =
        r\cdot c^{\widetilde{\xi}}_{\lozenge_B}(\lozenge_B)
        +c^{\widetilde{\xi}}_{N}(\lozenge_B)
        \geq r.
        \]

        Next we show the reverse inequality $c^{\widetilde{\xi}}_{\restr{M}{B}}(\lozenge_B)\leq r$.
        We break down the proof into the following steps.
        \begin{enumerate}
            \item First we observe that $s$ is the only source vertex of $B$.
        Suppose there exists an arrow from $a\in B$ to $s$ in $B$. 
        Then according to the definition of $B$, 
        there must exist a path from $s$ to $t$ passing through $a$.
        However, this would create a cycle containing $s$, 
        which contradicts the assumption that $G$ is acyclic.
        The uniqueness follows immediately from the definition of the convex hull.
        Similarly, $t$ is the only sink vertex of $B$.
        \item Consider the essential course $\widetilde{\xi}(B)\coloneqq (C,F)$, where $C$ is a connected quiver and $F\colon C_0\to B_0$ is the labeling map. Since this is an essential course of $B$ and $s,t$ are essential vertices of $B$, there exists vertices $c_s,c_t\in C_0$
        such that $F(c_s)=s$ and $F(c_t)=t$.
        As $C$ is connected, we can find a 
        type $\mathbb{A}_n$ subquiver of $C$
        starting from 
        $c_s$ and ending at $c_t$.
        The labeling map $F$ then induces a 
        type $\mathbb{A}_n$ subquiver of $B$
        starting from $s$ and ending at $t$.
        We denote this subquiver by $W$.
        For simplicity, we compose each subsequence of concatenable arrows in $W$ to a path,
        such that $W$ can be written in the form of head-to-head and tail-to-tail paths $p_l\cdots p_1$.
        Notice that both $W$ and $p$ can be viewed as essential courses on $B$.
        By the first point above, the start of $p_1$ is always $s$ and the target of $p_l$ is always $t$.
        In addition, since each consecutive two paths have opposite directions, it follows that $l$ must be an odd number.
        % thus we can write $W$ as $p_{2i+1}p_{2i}\cdots p_2 p_1$ for some $i\geq 0$.
        \item 
        We proceed with the proof by induction on $l$.
        For the base case $l=1$, we have
        \[
        \begin{aligned}
        c^{\widetilde{\xi}}_{\restr{M}{B}}(\lozenge_B)
        & =
        d_{\tour_{\widetilde{\xi}(B)}(\restr{M}{B})}\big[\tour_{\widetilde{\xi}(B)}(\restr{V_{B}}{B})\big]
        \\
        & \leq 
        d_{\tour_{W}(\restr{M}{B})}\big[\tour_{W}(\restr{V_{B}}{B})\big]\\
        & \mbox{\textcolor{yellow}{----------------}}\\
        & \leq 
        d_{\tour_{p_1}(\restr{M}{B})}\big[\tour_{p_1}(\restr{V_{B}}{B})\big]\\
        & =d_{\tour_{p}(\restr{M}{B})}\big[\tour_{p}(\restr{V_{B}}{B})\big]\\
        &=r,
        \end{aligned}
        \]
        where the penultimate equality follows from full commutativity.
        For the induction step, assuming the statement holds for $l=2i-1$,
        we consider $l=2i+1$.
        In this case, we have
        $W=p_{2i+1}p_{2i}\cdots p_2 p_1$, where the last two paths are of the form:
        \[
        \begin{tikzcd}
            \underset{t}{\bullet}&\underset{}{\bullet}\arrow[l,"p_{2i+1}"']\arrow[r,"p_{2i}"]&\underset{u}{\bullet}\arrow[ll,dashed, bend left,"\pi"]&\cdots\arrow[l].
        \end{tikzcd}
        %mirrored version
        % \begin{tikzcd}
        %    \cdots\arrow[r]
        %     &
        %     \underset{n}{\bullet}\arrow[rr,dashed, bend left,"\pi"]
        %     &
        %     \underset{}{\bullet}\arrow[r,"p_{2i+1}"']\arrow[l,"p_{2i}"]
        %     &
        %     \underset{t}{\bullet}.
        % \end{tikzcd}
        \]
        As $u$ is a vertex in $\Conv(\Set{s,t})$, 
        it lies on a path from $s$ to $t$, 
        and we can construct the dashed path denoted by $\pi$.
        By full commutativity, $M(p_{2i+1})=M(\pi)\circ M(p_{2i})$. 
        This implies that
        \[
        \begin{aligned}
            c^{\widetilde{\xi}}_{\restr{M}{B}}(\lozenge_B)
            & \leq 
            d_{\tour_{W}(\restr{M}{B})}\big[\tour_{W}(\restr{V_{B}}{B})\big]\\
            & = 
            d_{\tour_{p_{2i+1}p_{2i}p_{2i-1}p_{2i-2}\cdots p_2 p_1}(\restr{M}{B})}\big[\tour_{p_{2i+1}p_{2i}p_{2i-1}p_{2i-2}\cdots p_2 p_1}(\restr{V_{B}}{B})\big]\\
            & = 
            d_{\tour_{\pi p_{2i}p_{2i}p_{2i-1}p_{2i-2}\cdots p_2 p_1}(\restr{M}{B})}\big[\tour_{\pi p_{2i}p_{2i}p_{2i-1}p_{2i-2}\cdots p_2 p_1}(\restr{V_{B}}{B})\big]\\
            & \leq 
            d_{\tour_{\pi p_{2i-1}p_{2i-2}\cdots p_2 p_1}(\restr{M}{B})}\big[\tour_{\pi p_{2i-1}p_{2i-2}\cdots p_2 p_1}(\restr{V_{B}}{B})\big]\\
            & =
            d_{\tour_{(\pi p_{2i-1})p_{2i-2}\cdots p_2 p_1}(\restr{M}{B})}\big[\tour_{(\pi p_{2i-1})p_{2i-2}\cdots p_2 p_1}(\restr{V_{B}}{B})\big]\\
            & \leq 
            r.
        \end{aligned}
        \]
        The last inequality follows from the induction hypothesis,
        as $(\pi p_{2i-1})p_{2i-2}\cdots p_2 p_1$ 
        is a sequence of $2i-1$ head-to-head and tail-to-tail paths.
        \end{enumerate}

    Combining the two inequalities, we can conclude that $c^{\widetilde{\xi}}_{\restr{M}{B}}(\lozenge_B)=r$.
    This, along with (\ref{eq:compression-to-restricted-compression}),
    completes the proof.
    % \colorbox{yellow}{using rhombus here in the mind of the shape of maps.}
    \end{proof}
\end{lemma}


==> sec6/legacy_00621.tex <==

\subsubsection{Atomic Structure of Silica}\label{sec:silica}

\construction

For our initial example, we study the atomic arrangement of amorphous silica. 
Our dataset is a point cloud representing silicon and oxygen atoms in silica \cite{le2010isaacs}.
We apply the constant thinning model in \ref{subsec:model-point-cloud}, 
selectively removing atoms to disrupt the structured arrangement,
and subsequently employing connected persistence diagrams to evaluate the resulting impact on the atomic structure.

The figure below provides an illustrative representation of our input data, featuring highlighted chemical bonds. 
Notably, the structure displays visible ring formations.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.3\textwidth]{images/silica_input.jpg}
    \caption{Atomic representation of silica with illustrated chemical bonds. Blue points represent silicon atoms, while red balls represent oxygen atoms.
    %Notice the observable ring structures.
    }
    \label{fig:silica_input}
\end{figure}


\noindent\textbf{Case 1: Removal of All Silicon Atoms}

The first scenario evaluates how the topology changes in the absence of silicon atoms. We remove all silicon atoms while leaving the oxygen atoms in place.

\begin{figure}[H]
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{images/PD-silica-marked.png}
\caption{} \label{fig:example-silica-case1-a}
\end{subfigure}
\hspace*{\fill}
\begin{subfigure}{0.32\linewidth}
\centering
\includegraphics[width=\linewidth]{images/PD-silica-wo-marked.png}
\caption{} \label{fig:example-silica-case1-b}
\end{subfigure}
\hspace*{\fill}
\begin{subfigure}{0.32\linewidth}
\centering
\includegraphics[width=0.82\linewidth]{images/cPD-silica-1.png}
\caption{} \label{fig:example-silica-case1-c}
\end{subfigure}
\caption{
(a) Persistence diagram of the original atomic configuration.
(b) Persistence diagram of the oxygen atom-only configuration.
(c) Connected persistence diagram of the commutative ladder constructed from the two preceding states.
}
\label{fig:example-silica-case1}
\end{figure}

We highlight a collection of generators in Figure \ref{fig:example-silica-case1-a} and another collection in Figure \ref{fig:example-silica-case1-b}, both represent their prominent features \cite{hiraoka2016hierarchical}.
We observe that these generators seem to persist along the thinning process, 
but that cannot be justified by the standard persistence diagrams alone.
A connected persistence diagram can help us to confirm this observation,
where we focus on the previously highlighted ellipse regions and dimming out generators outside of them. 
Here, we find that most connecting lines originate from the ellipse region, 
further supporting our initial observation 
that the birth time of the main feature is delayed, with its basic structure maintained.

\noindent\textbf{Case 2: Thinning Out Oxygen Atoms at a 50\% Rate}

In the second scenario, oxygen atoms are removed at a 50\% rate, and silicon atoms remain intact.
\begin{figure}[H]
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{images/PD-silica-marked.png}
\caption{} \label{fig:example-silica-case2-a}
\end{subfigure}
\hspace*{\fill}
\begin{subfigure}{0.32\linewidth}
\centering
\includegraphics[width=\linewidth]{images/PD-silica-O-thinning.png}
\caption{} \label{fig:example-silica-case2-b}
\end{subfigure}
\hspace*{\fill}
\begin{subfigure}{0.32\linewidth}
\centering
\includegraphics[width=0.82\linewidth]{images/cPD-silica-2.png}
\caption{} \label{fig:example-silica-case2-c}
\end{subfigure}
\caption{
(a) Persistence diagram of the original atomic configuration.
(b) Persistence diagram of the configuration after a 50\% removal of oxygen atoms.
(c) Connected persistence diagram of the commutative ladder constructed from the two preceding states.
}
\label{fig:example-silica-case2}
\end{figure}

Unlike the first case, the primary topological feature undergoes noticeable deformation, and the transition distance is significantly longer. 
The connected persistence diagram reveals lines deviating from the main feature in Figure \ref{fig:example-silica-case2-b}
perpendicular to the diagonal line, corresponding to homology cycles whose affiliated oxygen atoms were retained during the thinning process. 
Moreover, the generators circled out in Figure \ref{fig:example-silica-case2-c}
do not originate from the main feature before thinning, they exhibit new birth times that precede those of the transformed main feature.

This comparative analysis highlights the different impacts of the removal rules applied. Even though the number of atoms removed is approximately the same in both scenarios, the second one exhibits more pronounced disruptions in the structure, as evidenced by the connected persistence diagrams. This illustrates the sensitivity and diagnostic power of the connected persistence diagrams in revealing topological changes within a structure.

